Spectral Networks and Non-abelianization

We generalize the non-abelianization of Gaiotto-Moore-Neitzke from the case of $SL(n)$ and $GL(n)$ to arbitrary reductive algebraic groups. This gives a map between a moduli space of certain $N$-shifted weakly $W$-equivariant $T$-local systems on an open subset of a cameral cover $\tilde{X}\rightarrow X$ to the moduli space of $G$-local systems on a punctured Riemann surface $X$. For classical groups, we give interpretations of these moduli spaces using spectral covers. Non-abelianization uses a set of lines on the Riemann surface $X$ called a spectral network, defined using a point in the Hitchin base. We show that these lines are related to trajectories of quadratic differentials on quotients of $\tilde{X}$. We use this to describe some of the generic behaviour of lines in a spectral network.

==> Non_Abelianization_Cameral.tex <==
%\section{Non Abelianization via Cameral Networks}
%\label{sec: flat Donagi Gaitsgory}

%\include{Non_Abelianization_Cameral.tex}

\subsection{Weakly equivariant bundles}



In this section, we will introduce some of the terminology used in \ref{item:abelian_data}. However, we are interested in a modified version of Donagi and Gaitsgory's result \cite{donagi2002gerbe}, mentioned in \ref{sec: cameral covers}.

\begin{theorem}
\label{thm:flat_DG}
Consider the unramified map $\pi : \tilde X \setminus R \to X \setminus P$, where we have removed the branch points and their preimages. Then there is an equivalence of categories between:
\begin{enumerate}
\item Weakly $W$-equivariant, $N$-shifted flat $T$-bundles $\cL$ on $\tilde X \setminus R$;
\item Flat $N$-bundles $\cE$ on $X \setminus B$, such that $\cE/T \cong \tilde X \setminus P$.
\end{enumerate}
\end{theorem}

This theorem is a modification of the following special case of Donagi and Gaitsgory's results:

\begin{theorem}[Special case of Theorem 6.4 of \cite{donagi2002gerbe}]
\label{thm: unramified donagi gaitsgory }
If $\tilde{X}\rightarrow X$ is an unramified map, then there is an equivalence of categories:
\[
\begin{tikzcd}
\{\text{$N$-bundles $E_{N}\rightarrow X$, with } E_{N}/T\cong \tilde{X} \}\arrow{d}{\cong} \\ \{\text{Weakly $W$-equivariant, $N$-shifted $T$-bundles on $\tilde{X}$}\}
\end{tikzcd}
\]
\end{theorem}

It is worth briefly mentioning how this theorem is proved.  The categories on both sides of the correspondence sheafify over $X$.  The local computation is trivial at points.  The map from the left hand side to the right hand side is given by considering $E_{N}\rightarrow E_{N}/T$ as a $T$-bundle.  We note that the weak $W$-equivariance is given by a lift of $w\in W$ to $N$, and we note that the $N$-action clearly maps to $\Aut_{X}(E_{N}\rightarrow E_{N}/T)$.  The reverse map is given by noting that the map $N\rightarrow \Aut_{X}(\cL)$, gives an $N$-action on fibers, and hence gives it the structure of an $N$-bundle over $X$.
\todo{This paragraph seems to be saying, more or less, what is said again a few pages later, in the proof of theorem \ref{thm:flat_DG}.}

Theorem \ref{thm:flat_DG} is the analogue of Theorem \ref{thm: unramified donagi gaitsgory } in the case of flat bundles.

We now introduce the necessary definitions for understanding the above theorems.

\begin{definition}
\label{def: Automorpshisms of T system  on X}
Let $\cL$ be a $T$-bundle on $\tilde{X}$.  We define:
\[
\Aut_{X}(\cL) = \{(w,\phi) | w\in W, \phi : w^*\cL \overset{\cong}{\to} \cL \}.
\]

\end{definition}

\todo{make clear that $\cL$ here refers to the bundle over $X$}

Note that this forms a sheaf on $X$.  Furthermore in the case that $\cL$ is a flat $T$-bundle there is a distinguised set of sections of this bundle which form a local system $\mathscr{Aut_{X}}(\cL)$ as follows:

\begin{definition}[The local system $\mathscr{Aut_{X}}(\cL)$]

Consider the functor 
\[Open_{X}\rightarrow Set\]
\[U\mapsto Aut^{flat}_{U}(\cL):=\{(w, \phi)|w\in W| \phi: w^{*}\Gamma(U,\cL)\overset{\cong}{\to} \Gamma(U,\cL),\}\]
where by $\Gamma(U,\cL)$ we mean the flat sections of $\cL$ on $U$.
\end{definition}

This is clearly a local system, because glocabl sections of $\cL$ form a local system.  We can consider this as giving a flat connection on the sheaf corresponding to $Aut_{X}(\cL)$ from definition \ref{def: Automorpshisms of T system  on X}.

\begin{remark}
Sections of the local system $\mathscr{Aut_{X}}(\cL)$ consists of the automorphisms which preserve the local system structure on $\cL$.
\end{remark}

\begin{definition}
\label{defin:weakly}
A \textbf{weakly $W$-equivariant} (flat)$T$ bundle on $\tilde{X}$, is a $T$-bundle $\cL$ on $\tilde{X}$, such that for every $w\in W$, there exists an isomorphism $w^{*}\cL\xrightarrow{\cong} \cL$. In other words, the natural projection $\Aut_X(\cL) \to W$ is surjective.
\end{definition}

When $\cL$ is a weakly $W$-equivariant $T$-bundle, there is a short exact sequence:
\begin{equation}
\label{eq:aut_not_split}
\begin{tikzcd}
1\arrow{r} & \Hom(\tilde X, T)\arrow{r} & \Aut_X(\cL) \arrow{r} & W\arrow{r} & 1 .
\end{tikzcd}
\end{equation}

When $\cL$ is a weakly $W$-equivariant flat $T$-bundle there is a short exact sequence

\begin{equation}
\label{eq:aut_not_split_flat}
\begin{tikzcd}
1\arrow{r} & \Hom_{lc}(\tilde X, T)\arrow{r} & \mathscr{Aut_X}(\cL) \arrow{r} & W\arrow{r} & 1 .
\end{tikzcd}
\end{equation}
where $Hom_{lc}(\tilde{X}, T)$ correspond to the homomorphisms which are constant on each connected component of $\tilde{X}$.

\begin{example}
\label{ex:w-equivariant}
Any $W$-equivariant $T$ bundle on $\tilde X$ is weakly $W$-equivariant. However, in Definition \ref{defin:weakly} we do \emph{not} require an action of $W$ on the $T$-bundle -- that is, we do not require a map $W\rightarrow \Aut_{X}(\cL)$. 

In fact, $W$-equivariant bundles are precisely those weakly $W$-equivariant bundles for which the sequence \ref{eq:aut_not_split} splits. In what follows, we will be interested instead in the case $\Aut_X(\cL) \cong N$, which is, in general, a non-trivial extension of $W$ by $T$.
\end{example}

\begin{definition}
A \textbf{weakly $W$-equivariant, $N$-shifted $T$ bundle} $\cL$ is a weakly $W$-equivariant $T$ bundle $\cL$, together with the data of a map $\gamma$ making the following diagram commute.
\begin{equation}
\label{diag:n_twisted}
\begin{tikzcd}
1 \arrow{r} \arrow{d} & T \arrow{r} \arrow{d}{\text{diag}} & N \arrow{r} \arrow{d}{\gamma} & W \arrow{r} \arrow{d}{1} & 1\arrow{d} \\
1 \arrow{r} & \Hom(\tilde{X},T) \arrow{r} & \Aut_{X}(\cL) \arrow{r} & W \arrow{r} & 1
\end{tikzcd}
\end{equation}
\end{definition}

%We denote by $\cM_{dR}^{W,N}(\tilde X,T)$ the moduli space of weakly $W$-equivariant, $N$-shifted flat $T$-bundles on $\tilde X$.

%Note that in the case $\cL$ is a local system, we can endow $\Aut_{X}(\cL)$ with the structure of a local system on $X\backslash P$.  One way to see this is that one can use the parallel transport on $\tilde{X}\rightarrow X$, and $\cL\rightarrow \tilde{X}$ along a path (avoiding branch points) from $x_{1}$ to $x_{2}$ to give a map $\Aut_{X}(\cL)|_{x_{1}}\rightarrow \Aut_{X}(\cL)_{x_{2}}$.  As the parallel transport on $\tilde{X}$ and $\cL$ only depends on the homotopy class of this path in $X\backslash P$, and hence this gives $\Aut_{X}(\cL)$ the strucutre of a local system on $X\backslash P$.

\begin{definition}
A \textbf{weakly $W$-equivariant, $N$-shifted flat $T$ bundle} $\cL$ is a weakly $W$-equivariant flat $T$ bundle $\cL$, together with the data of a map $\gamma$ making the following diagram commute
\begin{equation}
\label{diag:n_twisted}
\begin{tikzcd}
1 \arrow{r}\arrow{d} & T \arrow{r} \arrow{d}{\text{diag}} & N \arrow{r} \arrow{d}{\gamma} & W \arrow{r} \arrow{d}{1} & 1\arrow{d} \\
1 \arrow{r} & \Hom(\tilde{X},T) \arrow{r} & \Aut_{X}(\cL) \arrow{r} & W \arrow{r} & 1,
\end{tikzcd}
\end{equation}
and $\gamma(N)\in \Gamma(\mathscr{Aut_{X}})(\cL)\subset Aut_{X}(\cL)$.
\end{definition}

\begin{remark}
\label{remark: N-twisting at a point}
Note that we can define $N$-twisting data by just specifying 
\[\gamma_{x}: N\xrightarrow{\gammma} \Aut_{X}(\cL)|_{x} \]
at some point $x\in X$, provided that for each $a\in Im(\gamma)$, $a$ is invariant under the monodromy around any loop in $\pi_{1}(X,x)$.
\end{remark}

\begin{definition}
Suppose that we have a map $\gamma: N\xrightarrow{\gammma} \Aut_{X}(\cL)|_{x}$. Let $\rho(\sigma): \cL|_{x}\rightarrow \cL|_{x}$ be the monodromy of $\Tot(\cL)$ (considered as a sheaf over $X$) around a loop $\sigma \in \pi_{1}(X,x)$.
%define $n\in N$, as the element such that $\rho(p)= p\bullet \gamma(n)$.

Let $p\in \cL|_{x}$.
We say that the $(\gamma, \cL)$ is of \textbf{$N$-local type around $\sigma$}, if $\rho(\sigma)\big(p\bullet \gamma(n')\big)=\rho(\sigma)(p)\bullet \gamma(n')$, for all $n'\in N$. This does not depend on the choice of $p\in \cL_{x}$.
\end{definition}

\begin{proposition}
\label{prop: N local type requirement}
Suppose that $(\gamma, \cL)$ is of $N$-local type around $\sigma$ for all $\sigma \in \pi_{1}(X,x)$.  Then for each $a\in Im(\gamma)$, $a$ is invariant under the monodromy around any loop in $\pi_{1}(X,x)$, and hence by remark \ref{remark: N-twisting at a point} $\gamma$ defines $N$-shifting data for $\cL$.
\end{proposition}

\begin{remark}
We clearly need only require $(\gamma, \cL)$ is of $N$-local type around a set of $\sigma\in \pi_{1}(X,x)$ that generate $\pi_{1}(X,x)$.
\end{remark}

\begin{proof}[Proof of Proposition \ref{prop: N local type requirement}]
Let $\rho: \Aut_{X}(\cL)|_{x}\rightarrow \Aut_{X}(\cL)|_{x}$ be the monodromy around some loop $\sigma\in \pi_{1}(X,x)$.  Pick $p\in \cL|_{x}$.  Let $n\in N$ be defined by the requirement that $\rho(p)=p\bullet n_{2}$.

Then for any $n_{1}\in N$ we have (where $p\bullet n$ means $p\bullet \gamma(n)$)
\begin{align*}
    \rho^{-1}(\rho(p)\bullet n_{1}) &= \rho^{-1}(p \bullet n_{2}n_{1} )\\
    &= p \bullet n_{2}n_{1}((n_{1}^{-1}n_{2}^{-1})n_{2}^{-1}(n_{2}n_{1}))\\
    &= p \bullet n_{1}
\end{align*}
where we used the $N$-local type requirement in the second equality.
This calculation says that the map $\gamma$ is invariant under the monodromy generated by the loop in $\mathscr{Aut_{X}}(\cL)$.  The proposition follows.
\end{proof}

\begin{remark}
It will follow immediately from Theorem \ref{thm:flat_DG}, that the requirement of $N$-local type around all $\sigma\in \pi_{1}(X,x)$ is a necessary condition for $\gamma$ to extend to $N$-shifting data for $\cL$.
\end{remark}

%\todo{Check to work out whether I need some for of R-twisting! A: No -- because I am considering the case with no ramification.}

\todo{In the following do I need to specify tame ramification? -- yes somewhere need to note everything on punctured surfaces is tamely ramified.}

\todo{I am sure that I can and should prune some of the following-- not sure which at the moment}


\begin{definition}
We introduce the following notation.
\begin{itemize}
    \item We denote by $\Loc_{N}(X)$ the moduli space of flat $N$-bundles on a space $X$.
    \item We denote by $\Loc_{N}^{x}(X)$-the moduli space of flat $N$-bundles on $X$, trivialized at $x$.
    \item We denote by $\Loc_{N}^{\tilde{X}}(X)$ ($\Loc_{N}^{x, \tilde{X}}(X)$) the moduli space of flat $N$-bundles $\cL$ (trivialized at $x$) together with an isomorphism $\cL/T\cong \tilde{X}$.
    \item We denote by $\Loc_{N}^{\tilde{X},m}(X\backslash P)$  ($\Loc_{N}^{x, \tilde{X},m}(X \backslash P)$) the moduli space of flat $N$-bundles (trivialized at $x$) together with an isomorphism $\cL/W\cong \tilde{X}$ and such that for each type of singularity \todo{specify meaning} the monodromy around every instance of a fixed type is equal.
    \item We denote by $\Loc_{T}(X)$ ($\Loc_{T}^{x_{1},...,x_{n}}(X)$) the moduli space of flat $T$-bundles on $X$ (trivialized at $x_{1},...,x_{n}$.)
    \item We denote by $\Loc_{T}^{W,N}(\tilde{X})$ ($\Loc_{T}^{x_{1},...,x_{n}}(\tilde{X})$) the moduli space of $N$-shifted weakly $W$-equivariant flat $T$-bundles on $\tilde{X}$ (trivialized at $x_{1},...,x_{n}$).
    \item We denote by  $\Loc_{T}^{W,N,m}(\tilde{X})$ ($\Loc_{T}^{x_{1},...,x_{n}}(\tilde{X})$) the moduli space of $N$-shifted weakly $W$-equivariant flat $T$-bundles on $\tilde{X}$ (trivialized at $x_{1},...,x_{n}$), such that the monodromy (when considered as a local system over $X$) around each fixed type of singularity of $\tilde{X}\rightarrow X$ is equal at the different points where a singularity of this type occurs. \todo{Rewrite this so that it is clear [ie. what is a type of singularity], and can apply to when we've removed the branch points}
\end{itemize}
\end{definition}


\begin{example}[Consequences for $T$-monodromy]
\label{example: Consequences for T monodromy}
Consider the case where $G=SL(2)$, $X=\bbA^{1}_{z}$, and $\tilde{X}=\bbA^{1}_{y}$, with the map $\tilde{X}\rightarrow X$ given by $z\mapsto y^{2}$.

Then $\Loc_{N}^{\tilde{X}, x}(X \backslash \{0\})\xrightarrow{\cong} wT$, with the map taking a local system to its monodromy around $0$. 

Let $x_{1}, x_{2}$ be the preimages of $x\in X$  in $\tilde{X}$.   Suppose that $\cL$ is an $N$-shifted, weakly $W$-equivariant flat $T$ bundle on $\tilde{X}$.   Then the monodromy of $\cL$ considered as a $T$-local system on $\tilde{X}$ must be $-1$, because for all $g\in Im(wT)$, $g^{2}=-Id$.


%Now consider a $T$-bundle $\cL$ on $\tilde{X}$, equipped with a trivialization at $x_{1}$ and $x_{2}$.  

%Consider the $T^{2}\rtimes W$ monodromy $\rho$ of $\cL$ (considered as a local system on $X$) on going around $0$ in $X$. 

%If we have a map $N\xrightarrow{\gamma} \Aut_{X}(\cL)|_{x} \subset GL(\cL|_{x_{1}}\oplus \cL|_{x_{2}})$.

%Firstly note that the image of $N$ can be described by
%\[im(T)=T_{SL_{\cL|_{x_{1}}\oplus \cL|_{x_{2}}}}\hookrightarrow SL(\cL|_{x_{1}}\oplus \cL|_{x_{2}})\hookrightarrow GL(\cL|_{x_{1}}\oplus \cL|_{x_{2}})\]
%\todo{what do SL, GL mean? I think this should be replaced with appropriate subsets of $\Aut(\cL)$}
%that is, using the weak $W$-equivariance, and the a basis of $\cL|_{x_{1}}\oplus \cL|_{x_{2}}$, corresponding to a basis for $\cL_{x_{1}}$ and a basis of $\cL_{x_{2}}$, we can write
%\[im(T)= \{\left(\begin{matrix} a & 0\\ 0 & a^{-1}\end{matrix}\right)\in End(\cL|_{x_{1}}\oplus \cL|_{x_{2}})\}\].

%Again using the weak $W$-equivariance, and this basis we can describe 

%\[Im(wT)= \{\left(\begin{matrix} 0 & a\\ -a^{-1} & 0\end{matrix}\right)\in End(\cL|_{x_{1}}\oplus \cL|_{x_{2}})\}\].

%Using Proposition \ref{prop: N local type requirement} we see that for any $p\in \cL|_{x}$

%\[\rho(p)= pg \mathrm{for} g\in Im(wT).\]

%This means that the monodromy of $\cL$ considered as a $T$-local system on $\tilde{X}$ must be $-1$, because for all $g\in Im(wT)$, $g^{2}=-Id$.

% Note that it looks like I am using the naive version of imaging monodromy does not depend on base point -- however I am not!

Note that this corresponds to the condition on monodromy of the $\bbC^{\times}$ local systems considered on the spectral cover in \cite{gaiotto2013spectral}, though they take a different approach to handling this phenomenon by considering twisted local systems.
\end{example}



\begin{proof}[Proof of Theorem \ref{thm:flat_DG}]
Let $\cE$ be a flat $N$-bundle on $X$, then $\cE\rightarrow \cE/T\cong \tilde{X}$ is a flat $T$-bundle on $\tilde{X}$ (the $T$-action is specified by $T\hookrightarrow N$).  We have a natural map $N\rightarrow \Gamma(X,\mathscr{Aut_{X}}(\cE))$, that fits into a commutative diagram of the form of diagram \ref{diag:n_twisted}.

This has an inverse map, in that if we have a weakly $W$-equivariant, $N$-shifted flat $T$-bundle $\cL$ on $\tilde{U}$, then the map $N\rightarrow \Gamma(X,\mathscr{Aut_{X}}(\cL)$ allows us to consider it as a flat $N$-bundle.
\end{proof}

\begin{remark}[Monodromy Coordinates]
We can give (complex analytic) coordinates on $Loc^{N, x}, Loc^{N,x,\tilde{X}}$ and $Loc^{N,x,\tilde{X},m}$ (and hence also on the corresponding moduli spaces of $T$-local systems) by the monodromy of the $N$-local system around paths in $\pi_{1}(X\backslash B)$.

Note that if we are dealing with $\Loc^{N,x,\tilde{X}}$ or with $\Loc^{N,x,\tilde{X},m}$, each such monodromy is constrained to fall inside a particular $T$-coset in $N$. \todo{equivalent to T to some power}
\end{remark}



\subsubsection{Choices of $N$-shifting}
\todo{We may end up removing this. Either way, it's incomplete and can be skipped while reading.}

\begin{example}
\label{ex:shifts_SL2}
If $(\cL,\gamma)$ is a weakly $W$-equivariant, $N$-shifted flat $T$-bundle and $X$ is connected, there may be other $N$-shifted structures on the same underlying $W$-equivariant $T$-bundle $\cL$. Consider the case $G = SL_2(\C)$, so that $T \cong \C^\times$ and $W \cong \Z/2$. Then the possible $N$-shifts are the automorphisms of the extension $N$.
\[
\begin{tikzcd}
1 \arrow{r} & \C^\times \arrow{r} \arrow{d}{1} & N \arrow{r} \arrow{d}{\gamma_a} & \Z/2 \arrow{r} \arrow{d}{1} & 1 \\
1 \arrow{r} &\C^\times \arrow{r} & N \arrow{r} & \Z/2 \arrow{r} & 1
\end{tikzcd}
\]
Any automorphism $\gamma_a$ is determined by:
\[
\left( \begin{array} {cc}
0 & 1 \\ -1 & 0 
\end{array} \right)
\mapsto
\left( \begin{array} {cc}
0 & a \\ -a^{-1} & 0 
\end{array} \right)
\]
for some $a\in \C^\times$. In particular, the possible $N$-shifts are parametrized by $\C^\times$.
\end{example}

More generally, if $(\cL,\gamma)$ is a weakly $W$-equivariant $N$-shifted $T$-bundle and $X$ is connected, then the possible $N$-shifts $\gamma$ are given by automorphisms of the extension:
\begin{equation}
\label{eq:extension_N}
\begin{tikzcd}
1 \arrow{r} &T \arrow{r} & N \arrow{r} & W \arrow{r} & 1.
\end{tikzcd}
\end{equation}
The following lemma describes these.

\begin{lemma}
The automorphisms of \ref{eq:extension_N} are given by $(\C^\times)^r$, where $r = \rank(G)$, if $X$ is connected.
\end{lemma}
\todo{Perhaps we can see $(\C^\times)^r$ more canonically, as maximal torus modulo center.}

\begin{proof}
Automorphisms of \ref{eq:extension_N} must be the identity on $T$, so they are determined by their action on a representative from each coset of $T$ in $N$. 
\begin{itemize}
    \item Consider first cosets $s_{\alpha}T$, where $s_{\alpha}$ is a reflection in $W$ associated to a simple root $\alpha$. The action on each of these reduces to the case of $SL_2(\C)$, treated in Example \ref{ex:shifts_SL2}. \todo{up to some $\pm$} There are $r$ simple roots, which gives $(\C^\times)^r$.
    \item The action of an automorphism on $\{s_{\alpha}T\}_{\alpha \text{simple}}$ determines the action on all other cosets, by decomposing any $w\in W$ into simple reflections. We need to prove that the automorphisms of $s_{\alpha}T$ satisfy the Coxeter relations. \todo{Write case bash or find good proof} 
\end{itemize}
\end{proof}

\subsubsection{The S-monodromy condition}

Non-abelianization does not work if we allow arbitrary $N$-monodromy around points $p\in P$ (see remark \ref{remark: restriction of T monodromy to T_alpha} to see why).  The purpose of this section is to show that certain substacks of the stacks in Theorem \ref{thm:flat_DG} correspond to each other.

\begin{definition}
$Loc_{T}^{W,N,\alpha,-1, x}(\tilde{X}\backslash R)$ is the substack of $Loc_{T}^{W,N, \tilde{x}_{1},...,\tilde{x}_{|W|}}(\tilde{X}\backslash R)$, corresponding to local systems such that 
\begin{itemize}
\item If we consider the monodromy of this considered as a local system around $X$, for any path lifting the loop around $p\in P$ gives a map $E_{T}|_{\tilde{x}_{i}}\rightarrow E_{T}|_{\tilde{x}_{j}}$.  Using the trivializations this can be identified as an element of $T$.  We require it to be in $T^{\alpha}$, where $\alpha$ is the root such that 
\[\tilde{X}\hookrightarrow \ft_{K_{X}(Q)}\xrightarrow{\alpha} tot(K_{X}(Q))\] is singular on the locally connnected component of $\tilde{X}$.\todo{specify better}
\end{itemize}
\end{definition}

\begin{remark}
This means that the monodromy $\gamma_{r}$ around $r\in R$, is given by $\gamma_{r}=i(-1)$, where 
\[i:\bbC^{\times}\hookrightarrow T\]
maps $\bbC^{\times}\cong T^{\alpha}\hookrightarrow T$, where $\alpha$ is the root such that 
\[\tilde{X}\hookrightarrow \ft_{K_{X}(Q)}\xrightarrow{\alpha} tot(K_{X}(Q))\] is singular at $r$.
\end{remark}

\todo{prior to this definition I need the definition of $T^{\alpha}$, and a choice of loop around each point.  Matei: I think you've written this so just tell me where to reference it. Benedict: look at lemma \ref{lem:torus_decomposition} and the paragraph preceding it}

\begin{definition}
\label{defin:N_alpha_monodromy}
$Loc_{N}^{\tilde{X}, \alpha}(X\backslash P)$ is the substack of $Loc_{N}(X\backslash P)$, such that the monodromy around each $p\in P$ is contained in $N_{SL(2)}\rightarrow{f} N$, for $f$ defined as follows:
\begin{itemize}
    \item Pick a trivialization of the cameral cover.  This determines a branch identified with $1\in W$.  On this branch some root $\alpha$ vanishes at $p$.
    \item Take the map $\rho_{\alpha}:SL_{2}\rightarrow G$, and note that it gives a map $N_{SL_{2}}\rightarrow N_{G}$. \todo{prove that the image is inside $N_{G}$, or otherwise}
    \item Take local systems such that the monodromy around $p$ is contained in $N_{SL_{2}}$.
\end{itemize}
\end{definition}

\begin{remark}
This is well-defined. \todo{Check this -- especially in the non simply laced case.}
\end{remark}

\todo{I clearly have a problem here because in the second definition but not the first I need a trivialization}

\begin{conjecture}
\ref{Thm: flat DG restricted monodromy}
There is a commutative diagram
\[
\begin{tikzcd}
\Loc_{T}^{W,N,\alpha,-1}(\tilde{X}\backslash R) \arrow{r} \arrow{d}{\rho|_{\Loc_{T}^{W,N,\alpha,-1}(\tilde{X}\backslash R)}}&  \Loc_{T}^{W,N}(\tilde{X}\backslash R) \arrow{d}{\rho}\\
\Loc_{N}^{\tilde{X}, \alpha}(X\backslash P) \arrow{r} & \Loc^{\tilde{X}}_{N}(X\backslash P)
\end{tikzcd}
\]
with both vertical arrows being isomorphisms.
\end{conjecture}

\begin{proof}
Given that in Theorem \ref{thm:flat_DG} we proved that the vertical arrow on the right hand side was an equivalence, we merely need to show that the two restrictions on monodromy correspond to each other under the non-abelianization map.

This is clear from the earlier discussion of how $N$-mopnodromy relates to $T$-monodromy.
\todo{Check this -- maybe give more details}
\end{proof}


\begin{remark}
\label{remark: restriction of T monodromy to T_alpha}
The reason we restrict to $T$-bundles with monodromy inside $T_{\alpha}$ is because of the relation between cameral covers and spectral covers \cite{donagi1993decomposition}, which we consider in section \ref{sec: Spectral Decomposition}.  Essentially we need this condition in order for there to be a map from $Loc_{T}^{W,N}(\tilde{X}\backslash R)\rightarrow Loc_{\bbC^{\times}}(X_{\lambda}^{pn}\backslash R_{\lambda})$.  That is, it is non abelianization on these $T$-bundles that will correspond to non-abelianization where we consider associated vector bundles rather than principal $G$-bundles.
\end{remark}



==> S3_setaside.tex <==
\section{Lie theoretic preliminaries}
\label{sect:prelim}

This section contains some Lie theoretic notation and constructions, which will be referenced in other sections. There are no novel ideas in this section, and it can be safely skipped until you encounter back-references to it. Note that Warning \ref{warn:sl2_triples} outlines a non-standard sign convention for Chevalley bases, which we use throughout the paper.


\subsection{Chevalley bases}

We begin by fixing a basis of $\fr g$ with respect to which the structure constants are particularly well behaved.

\begin{definition}
\label{defin:chevalley_basis}
Let $\fr g$ be a complex semisimple Lie algebra. Fix a Cartan $\fr t \subset \fr g$, which determines a root space decomposition $\fr g = \fr t \oplus \bigoplus_{\alpha \in \Phi} \fr g_\alpha$; also fix a set of simple roots.
Consider a basis\footnote{We mean a basis of the underlying vector space.} of $\fr g$ compatible with this decomposition:
\begin{itemize}
    \item a basis $\{h_\alpha\}_{\alpha \text{ simple}}$ for $\fr t$;
    \item a basis $\{e_\alpha\}$ for each of the 1-dimensional root spaces $\fr g_\alpha$.
\end{itemize}
If $\gamma \in \Phi$ is not simple, write it as a linear combination of simple roots $\alpha_i$, and define $h_\gamma$ as the corresponding linear combination of the $h_{\alpha_i}$.

We call the basis a \textbf{Chevalley basis}\footnote{See warning \ref{warn:sl2_triples}.} if it satisfies the relations:
\begin{align}
    [h_\alpha, e_\gamma] &= 2 \frac{(\alpha, \gamma)}{(\alpha,\alpha)} e_\gamma,
    \label{eq:chevalley_sl2}
    \\
    [e_{\alpha}, e_{-\alpha}] &= -h_\alpha ,
    \label{eq:chevalley_cmm}
    \\
    \label{eq:chevalley_p}
    [e_\alpha, e_\gamma] &= \left\{
    \begin{array}{ll}
    0 & \text{if } \alpha + \gamma \text{ not a root,} \\
    \pm (p_{\alpha,\gamma}+1) e_{\alpha + \gamma} & \text{if } \alpha + \gamma \text{ is a root.}
    \end{array}
     \right.
\end{align}
In equation \ref{eq:chevalley_p}, $p_{\alpha,\gamma}$ is the largest integer such that $\alpha - p_{\alpha,\gamma} \gamma$ is a root. 
\end{definition}

\begin{remark}
\label{rem:describe_p}
If we want to fix numbers $C_{\alpha, \gamma}$ such that the system of equations:
\[
[e_\alpha, e_\gamma] = C_{\alpha,\gamma}\cdot e_{\alpha + \gamma}
\]
in the variables $\{e_{\gamma}\}_{\gamma \in \Phi}$ is consistent, it's not necessarily possible to take all $C_{\alpha, \gamma} = \pm 1$. Indeed, one can prove that $C_{\alpha, \gamma} C_{-\alpha, -\gamma} = (p_{\alpha, \gamma} + 1)^2$.

A Chevalley basis is appealing because it has $C_{\alpha, \gamma} = C_{-\alpha, -\gamma} = \pm (p_{\alpha, \gamma} + 1)$, which are small integers:
\begin{itemize}
    \item For $\fr g$ of type ADE, all $p_{\alpha, \gamma} = 0$.
    \item For $\fr g$ of type BCF, $p_{\alpha, \gamma} = 1$ if $\alpha, \gamma$ are both short roots, and $p_{\alpha, \gamma} = 0$ otherwise.
    \item For $\fr g = \fr g_2$, $p_{\alpha, \gamma} \in \{0,1,2\}$, depending on the angle between $\alpha$ and $\gamma$.
\end{itemize}
\end{remark}

\begin{warning}
\label{warn:sl2_triples}
According to our definition, for any root $\alpha$, $\{h_\alpha, e_\alpha, -e_{-\alpha}\}$ is an $\fr{sl}_2$ triple. However, the standard definition of a Chevalley basis does not include the minus sign in equation \ref{eq:chevalley_cmm}, which would make $\{h_\alpha, e_\alpha, e_{-\alpha}\}$ an $\fr{sl}_2$ triple. We chose a non-standard sign convention in order to simplify later constructions.
\end{warning}

Due to \ref{rem:describe_p} and \ref{warn:sl2_triples}, we can informally see a Chevalley basis as a choice of $\fr{sl}_2$ triples for all roots of $\fr g$, with brackets as simple as possible.


\begin{proposition}
Every complex semisimple $\fr g$ admits a Chevalley basis.
\end{proposition}

This result was proved by Chevalley in \cite{chevalley1955}, and a good exposition is given by Tao in the blog post \cite{tao_blog_chevalley}.

\begin{comment}
This is the proof sketch, keeping it around in case we decide to use it.

\begin{enumerate}
    \item Use the Killing form to identify $\fr h$ with $\fr h^\vee$, and define $h_{\alpha}$ as the co-roots with the normalization:
    \[  h_{\alpha} = \frac{2}{(\alpha,\alpha)} \alpha^\vee.   \]
    This ensures that \ref{eq:chevalley_sl2} holds.
    \item Take arbitrary generators for the root spaces and rescale them such that \ref{eq:chevalley_cmm} holds.
    \item We can still rescale $e_\alpha$ by some $A_\alpha$, as long as we rescale $e_{-\alpha}$ by $A_\alpha^{-1}$, so that \ref{eq:chevalley_cmm} is preserved. We can use this freedom to ensure that $C_{\alpha,\beta} = C_{-\alpha,-\beta}$. For this, we use the automorphism $\Phi$ of $\fr g$ which acts by $-1$ on $\fr h$, and on the root space by $\alpha \mapsto - \alpha$. Then $\Phi(e_\alpha) = b_\alpha e_\alpha$ for some $b_\alpha$, and we take $A_{\alpha}$ such that $A_\alpha = b_\alpha A_{-\alpha}$.
\end{enumerate}
\end{comment}



\begin{example}
\label{eg:chevalley_basis}
Let $\fr g = \fr{sl}_3$, and $\alpha, \beta$ denote a choice of simple roots. We construct a Chevalley basis from the following basis of the Cartan: 
\[
h_{\alpha} = \left(
\begin{array} {ccc}
1 & 0 & 0 \\
0 & -1 & 0 \\
0 & 0 & 0
\end{array}
\right)
\hspace{1cm}
h_{\beta} = \left(
\begin{array} {ccc}
0 & 0 & 0 \\
0 & 1 & 0 \\
0 & 0 & -1
\end{array}
\right)
\]
and the following basis vectors for the root spaces:
\[
e_{\alpha} = \left(
\begin{array} {ccc}
0 & 1 & 0 \\
0 & 0 & 0 \\
0 & 0 & 0
\end{array}
\right)
\hspace{1cm}
e_{\beta} = \left(
\begin{array} {ccc}
0 & 0 & 0 \\
0 & 0 & 1 \\
0 & 0 & 0
\end{array}
\right)
\hspace{1cm}
e_{\alpha + \beta} = \left(
\begin{array} {ccc}
0 & 0 & 1 \\
0 & 0 & 0 \\
0 & 0 & 0
\end{array}
\right)
\]
\[
e_{-\alpha} = \left(
\begin{array} {ccc}
0 & 0 & 0 \\
-1 & 0 & 0 \\
0 & 0 & 0
\end{array}
\right)
\hspace{7mm}
e_{-\beta} = \left(
\begin{array} {ccc}
0 & 0 & 0 \\
0 & 0 & 0 \\
0 & -1 & 0
\end{array}
\right)
\hspace{7mm}
e_{-\alpha - \beta} = \left(
\begin{array} {ccc}
0 & 0 & 0 \\
0 & 0 & 0 \\
-1 & 0 & 0
\end{array}
\right)
\]
There are other Chevalley bases for $\fr{sl}_3$.
For any re-scaling of $e_\alpha, e_\beta$ by $A, B \in \C^\times$, it is possible to re-scale $e_{\alpha + \beta}$ by $AB$, and $e_{-\alpha}, e_{-\beta}, e_{-\alpha - \beta}$ by $A^{-1}, B^{-1}, A^{-1}B^{-1}$, respectively, so that relations \ref{eq:chevalley_sl2} - \ref{eq:chevalley_p} are unchanged.
\end{example}

The existence of Chevalley bases implies the following fact, which will be used repeatedly.

\begin{lemma}
\label{lem:roots_commutators_vanish}
Let $\fr g$ be a semisimple Lie algebra, and consider a root space decomposition $\fr g = \fr t \oplus \bigoplus_{\alpha \in \Phi} \fr g_\alpha$, as in Definition \ref{defin:chevalley_basis}. Then for all $\alpha, \beta \in \Phi$ such that $\alpha+\beta \neq 0$, $[\fr g_\alpha, \fr g_\beta] \subset \fr g_{\alpha + \beta}$. Moreover, $[\fr g_\alpha, \fr g_\beta] = 0$ if and only if $\alpha + \beta \not \in \Phi$.
\end{lemma}

\begin{proof}
The root spaces $\fr g_\alpha$ are 1-dimensional, so it suffices to consider the bracket $[e_\alpha, e_\beta]$ for some $e_\alpha \in \fr g_\alpha$ and $e_\beta \in \fr g_\beta$. The Jacobi identity implies that, for all $h \in \fr t$:
\begin{align*}
\big[h, [e_\alpha,e_\beta] \big] &= \big[ [h,e_\alpha], e_\beta \big] + \big[ e_\alpha, [h,e_\beta] \big]
\\
&= \big[ \alpha(h)\cdot e_\alpha, e_\beta\big] + \big[e_\alpha, \beta(h)\cdot e_\beta\big]
\\
&= (\alpha + \beta)(h) \cdot [e_\alpha, e_\beta].
\end{align*}
Hence $[\fr g_\alpha, \fr g_\beta] \subset \fr g_{\alpha+\beta}$.

It's clear then that if $\alpha+\beta \not \in \Phi$, then $[\fr g_\alpha, \fr g_\beta] = 0$. The converse follows from the existence of a Chevalley basis: according to relation \ref{eq:chevalley_p}, if $\alpha + \beta$ is a root, then $[e_\alpha, e_\beta]$ is a nonzero scalar multiple of $e_{\alpha+\beta}$.
\footnote{For a more elementary proof of the converse, see e.g. Theorem 6.44 in \cite{kirillov_introduction}.}
\end{proof}

We now let $\fr g$ be a reductive Lie algebra. We fix a Chevalley basis for the semisimple part of $\fr g$.\footnote{Note that the root systems of $\fg$ and of its semisimple part are isomorphic.}
In particular, this determines a map:
\begin{align*}
    \Phi & \to \{\fr{sl}_2 \text{-triples in } \fr g \},
    \\
    \alpha &\mapsto (h_\alpha, e_\alpha, -e_{-\alpha}).
\end{align*}
In other words, each $\alpha$ determines a map $i_\alpha : \fr{sl}_2 \to \fr g$. Because $SL(2)$ is simply connected, Lie's theorems provide unique group homomorphisms $I_\alpha$, making the following diagram commute:

\begin{equation}
\label{diag:exp}
\begin{tikzcd}
\fr{sl}_2 \arrow{r}{i_\alpha}\arrow{d}{\exp} & \fr g \arrow{d}{\exp} \\
SL(2)\arrow{r}{I_\alpha} & G 
\end{tikzcd}
\end{equation}

Let $s_\alpha \in W$ be the reflection about the root hyperplane orthogonal to $\alpha$, and recall the short exact sequence
\begin{equation}
\label{eq:weyl_exact_seq}
\begin{tikzcd}
1 \arrow{r} & T \arrow{r} & N \arrow{r}{p} & W \arrow{r} & 1.
\end{tikzcd}
\end{equation}

Any $\fr{sl}_2$ triple, in particular the one coming from our Chevalley basis, determines an $n_\alpha \in N$ such that $p(n_\alpha) = s_\alpha$, via the formula:
\begin{equation}
\label{eq:preferred_lift}
n_\alpha := \exp \frac{\pi}{2} (e_\alpha + e_{-\alpha}).
\end{equation}

\begin{warning}
However, note that the lifts $n_\alpha$ do \emph{not}, in general, provide a section of $p: N \to W$. For instance, $n_\alpha^2 \neq \id$ in the setting of example \ref{ex:lift_sl2}. Providing a section of $p$ is impossible in general, because the sequence \ref{eq:weyl_exact_seq} does not split, for groups such as $SL(2n,\C)$.
\end{warning}


\begin{example}
\label{ex:lift_sl2}
For $\fr g = \fr{sl}_2$, a Chevalley basis is:
\[
h_\alpha = \left( \begin{array}{cc}
  1   & 0 \\
  0   & -1
\end{array}
\right)
\hspace{1cm}
e_\alpha = \left( \begin{array}{cc}
  0   & 1 \\
  0   & 0
\end{array}
\right)
\hspace{1cm}
e_{-\alpha} = \left( \begin{array}{cc}
  0   & 0 \\
  -1   & 0
\end{array}
\right).
\]
The corresponding lift is a rotation by $\pi/2$:
\[
n_\alpha = \exp \frac{\pi}{2} \left( \begin{array}{cc}
  0   & 1 \\
  -1   & 0
\end{array}
\right) = \left( \begin{array}{cc}
  0   & 1 \\
  -1   & 0
\end{array}
\right).
\]
\end{example}


 
\begin{lemma}
\label{lem:w}
$n_\alpha$ is a lift to $N$ of the simple reflection $s_\alpha$.
\end{lemma}

\begin{proof}
We prove that conjugation by $n_\alpha$ fixes $\fr t$, and its restriction to $\fr t$ is reflection about the hyperplane $\Ker \alpha$.
For this, we use the decomposition $\fr t = \langle h_\alpha\rangle_{\C} \oplus \Ker \alpha$, and treat two cases separately.
\begin{enumerate}
    \item We show that $n_\alpha h_\alpha n_\alpha^{-1} = - h_\alpha$. For $G = SL(2)$ and the standard $\fr{sl}_2$ triple $(h,e,f)$, this is a trivial computation. The general case is reduced to the $SL(2)$ case using diagram \ref{diag:exp}:
    \begin{align*}
        n_\alpha h_\alpha n_\alpha^{-1}
        &= \left.\frac{d}{dt}\right|_{t=0}
        e^{i_\alpha(\pi(e-f)/2)} 
        e^{i_{\alpha}(t h)}
         e^{i_\alpha(-\pi(e-f)/2)}  \\
        &= \left.\frac{d}{dt}\right|_{t=0}
        I_\alpha  \left(  e^{\pi(e-f)/2} 
        e^{t h}
         e^{-\pi(e-f)/2}\right) \\
         &= I_\alpha \left(  e^{\pi(e-f)/2} 
        h
         e^{-\pi(e-f)/2}\right) \\
         &= -h_\alpha .
    \end{align*}
    \item If $\alpha(h) = 0$, then:
    \[   
    [h, e_{\pm\alpha}] =\pm \alpha(h) e_{\pm\alpha} = 0.
    \]
    It follows that $n_\alpha h n_\alpha^{-1} = h$.

\end{enumerate}
\end{proof}

The next result is the main input for Lemma \ref{lemma: monodromy to Stokes factors}, where we interpret the LHS as a product of Stokes factors, and the RHS as the monodromy of an $N$-local system.

\begin{lemma}
\label{lem:triple_product}
We have the following identity in $G$:
\[   \exp{(e_\alpha)} \exp{(e_{-\alpha})}\exp{(e_\alpha)} = n_\alpha .  \]
\end{lemma}

\begin{proof}
Again, it suffices to prove this for $G=SL(2)$, because diagram \ref{diag:exp} means the general case follows from this one. For $SL(2)$ this is the straightforward identity:
\[   
\left( \begin{array}{cc}
    1 & 1  \\
    0 & 1
\end{array}
\right)
\left( \begin{array}{cc}
    1 & 0  \\
    -1 & 1
\end{array}
\right)
\left( \begin{array}{cc}
    1 & 1  \\
    0 & 1
\end{array}
\right)
=
\left( \begin{array}{cc}
    0 & 1  \\
    -1 & 0
\end{array}
\right).
\]
\end{proof}

Finally, for every root $\alpha$, the Killing form of $\fr g$ determines an orthogonal decomposition:
\begin{equation}
\label{eq:decomp_lie_algebra}
 \fr{t} = \fr t_{\alpha} \oplus \fr t_{\Ker(\alpha)} . 
\end{equation}  
Here $\fr{t}_\alpha = \langle h_\alpha \rangle_{\C}$; by construction, $h_\alpha$ is a scalar multiple of the co-root $\alpha^\vee$, the dual of $\alpha$ under the Killing form.

Let $T_{\alpha} = \exp (\fr t_{\alpha})$ and $T_{\Ker(\alpha)} = \exp (\fr t_{\Ker \alpha})$. We can equivalently describe $T_{\alpha}$ as the image $ I_{\alpha}(T_{SL(2)})$, under the homomorphism from diagram \ref{diag:exp}, of the maximal torus of $SL(2)$.

\begin{lemma}
\label{lem:torus_decomposition}
The multiplication homomorphism:
\[
T_{\alpha} \times T_{\Ker(\alpha)} \to T
\]
is surjective, and its kernel is contained in the subgroup:
\[
\big\{(\id, \id), \big(I_\alpha(-\id_{SL(2)}), I_\alpha(-\id_{SL(2)})\big)\big\}.
\]
\end{lemma}


\begin{proof}
Due to the orthogonal decomposition \ref{eq:decomp_lie_algebra} at the Lie algebra level, there is a surjective homomorphism $T_{\alpha} \times T_{\Ker \alpha} \to T$. Its finite kernel is the intersection $T_{\alpha} \cap T_{\Ker \alpha}$. Since $T_{\alpha} = I_\alpha(T_{SL(2)})$, and $T_{\Ker \alpha} \subset \Ker(\exp(\alpha))$, we need only analyze the diagram:
\[
\begin{tikzcd}
T_{SL(2)} \arrow{r}{I_{\alpha}} & T \arrow{r}{\exp(\alpha)} & \C^\times .
\end{tikzcd}
\]
It follows that:
\[    T_{\alpha} \cap T_{\Ker \alpha} \subset  I_{\alpha}\big(\Ker (\alpha\circ I_\alpha)\big). \]

Denote $\exp(\alpha_{SL(2)}) = \exp(\alpha) \circ I_\alpha$;
so it suffices to show that $\Ker \exp (\alpha_{SL(2)}) = \{ \pm \id_{SL(2)} \}$. $\Ker \exp( \alpha_{SL(2)})$ consists of the elements of $T_{SL(2)}$ whose adjoint action fixes $e_{\alpha_{SL(2)}}$; the latter is either:
\[
\left(\begin{array}{cc}
   0  & 1 \\
   0  & 0
\end{array} \right)
\text{    or    }
\left(\begin{array}{cc}
   0  & 0 \\
   -1  & 0
\end{array} \right).
\]
Either way, $\{\pm \id_{SL(2)}\}$ are the only elements of $T_{SL_2}$ whose adjoint action fixes it.
\end{proof}


\begin{lemma}
\label{lem:commutation_t_alpha}
For every $t\in T_\alpha \cong T_{SL_2}$, conjugation by $n_\alpha$ acts as a permutation:
\[
n_\alpha^{-1} t n_\alpha =  t^{-1}.
\]
\end{lemma}

\begin{proof}
The relation is the image under $I_\alpha$ of the $SL(2)$ relation:
\[
\left( \begin{array} {cc} 
a & 0 \\ 0 & a^{-1}
\end{array} \right)
\left( \begin{array} {cc} 
0 & 1 \\ -1 & 0
\end{array} \right)
=
\left( \begin{array} {cc} 
0 & 1 \\ -1 & 0
\end{array} \right)
\left( \begin{array} {cc} 
a^{-1} & 0 \\ 0 & a
\end{array} \right) .
\]
\end{proof}


\begin{lemma}
\label{lem:t_ker_comm}
The adjoint action of $T_{\Ker(\alpha)}$ on $\fr g$ fixes $e_{\pm \alpha}$. Consequently, the adjoint action of $T_{\Ker(\alpha)}$ on $T$ fixes $n_\alpha$.
\end{lemma}

\begin{proof}
If $h \in \fr t_{\Ker \alpha}$, then $[h,e_\alpha] = \alpha(h) e_\alpha = 0$. It follows that $\ad_{\exp(h)}(e_\alpha) = e_\alpha$.
\end{proof}


\begin{lemma}
\label{lem:adj_scalar}
For all $t \in T$, $\ad_t(e_\alpha)$ is a scalar multiple of $e_\alpha$. Moreover, all scalar multiples of $e_\alpha$ arise in this way.
\footnote{Note that, due to Lemma \ref{lem:t_ker_comm}, we could just as well restrict to $t\in T_\alpha$.} 
\end{lemma}

\begin{proof}
Consider relation \ref{eq:chevalley_sl2} from the Definition \ref{defin:chevalley_basis} of a Chevalley basis:
\[
[h_\gamma, e_\alpha] = 2 \frac{(\gamma, \alpha)}{(\gamma, \gamma)} e_\alpha .
\]
Using ad-invariance of the Lie bracket, and the fact that $\ad_{t}(h_\gamma) = h_\gamma$, we obtain:
\[
[h_\gamma,\ad_t(e_\alpha)] = 2 \frac{(\gamma, \alpha)}{(\gamma, \gamma)} \ad_t(e_\alpha) .
\]
Thus, $\ad_t(e_\alpha)$ belongs to the same root eigenspace as $e_\alpha$. Since the root eigenspaces are 1-dimensional, there exists $\lambda \in \C^\times$ such that:
\begin{equation}
\label{eq:adj_scalar}
\ad_t(e_\alpha)= \lambda e_\alpha.
\end{equation}

For the converse statement, it suffices to find, for every $\lambda \in \C^\times$, some $t_\lambda \in T_\alpha$ satisfying equation \ref{eq:adj_scalar}. Looking at the image of $T_{SL(2)}$ under $I_\alpha : SL(2) \to G$ reduces this to a simple computation in $SL(2)$. Choose any square root of $\lambda$, and then:
\[
\left(
\begin{array}{cc}
    \lambda^{1/2} & 0 \\
    0 & \lambda^{-1/2}
\end{array}
\right)
\left(
\begin{array}{cc}
    0 & 1 \\
    0 & 0
\end{array}
\right)
\left(
\begin{array}{cc}
    \lambda^{-1/2} & 0 \\
    0 & \lambda^{1/2}
\end{array}
\right)
=
\left(
\begin{array}{cc}
    0 & \lambda \\
    0 & 0
\end{array}
\right)
\]
\end{proof}


\begin{lemma}
\label{lem:commutation_n}
Let $n \in N$, and $[n] \in W$ is image in the Weyl group. Define $\alpha' = [n](\alpha)$. Then there exists some $t \in T_{\alpha'}$ such that:
\begin{itemize}
    \item $\ad_n(e_{\pm\alpha}) = \ad_t (e_{\pm \alpha'})$;
    \item $\Ad_{n} (n_\alpha) = \Ad_{t} (n_{\alpha'})$.
\end{itemize}
\end{lemma}

\begin{proof}
%\todo{MI: edited this proof 1/16; review. BM: Reviewed: 1/17}  
For all $\gamma \in \Phi$ and $h_\gamma$ as in Definition \ref{defin:chevalley_basis}, let $\gamma' = [n](\gamma)$. Due to Lemma \ref{lem:w}, $\ad_n(h_\gamma) = h_{\gamma'}$. Then, using $\ad$-invariance of the Lie bracket, relation \ref{eq:chevalley_sl2} from Definition \ref{defin:chevalley_basis} implies:
\[
[h_{\gamma'} , \ad_n(e_{\pm \alpha})] = \pm 2 \frac{(\gamma, \alpha)}{(\alpha, \alpha)} \ad_n(e_{\pm \alpha}).
\]
Similarly,
\[
[h_{\gamma'} , e_{\pm \alpha'}] = \pm 2 \frac{(\gamma', \alpha')}{(\alpha', \alpha')} e_{\pm \alpha'}.
\]

The bilinear pairing between roots is Weyl-invariant, so for all roots $\gamma$:
\[
\frac{(\gamma, \alpha)}{(\alpha, \alpha)} = \frac{(\gamma', \alpha')}{(\alpha', \alpha')}.
\]
Then $\ad_n(e_{\pm \alpha})$ and $e_{\pm \alpha'}$ belong to the same eigenspace for the adjoint action of $\fr t$.
These eigenspaces are one dimensional, which means $\ad_n(e_{\pm \alpha})$ and $e_{\pm \alpha'}$ are scalar multiples of each other.
Now, using Lemma \ref{lem:adj_scalar}, there exist $t_{\pm} \in T$ such that $\ad_n(e_{\pm \alpha}) = \ad_{t_{\pm}}(e_{\pm \alpha'})$. Moreover, due to Lemma \ref{lem:t_ker_comm}, we can assume that $t_{\pm} \in T_{\alpha'}$. To conclude, it remains to show that we can take $t_+ = t_-$.

We claim that $\ad_{t_+}(e_{-\alpha'}) = \ad_{t_-}(e_{-\alpha'})$.
Using the $\ad$-invariance of relation \ref{eq:chevalley_cmm} from Definition \ref{defin:chevalley_basis}, and applying $\ad_n$, we obtain:
\[
[\ad_{t_+}(e_{\alpha'}), \ad_{t_-}(e_{-\alpha'})] = - h_{\alpha'}.
\]
On the other hand, applying $\ad_{t_+}$ we obtain:
\[
[\ad_{t_+}(e_{\alpha'}), \ad_{t_+}(e_{-\alpha'})] = - h_{\alpha'}.
\]
Since $\ad_{t_+}(e_{-\alpha'})$ is a scalar multiple of $\ad_{t_-}(e_{-\alpha'})$, these two relations imply they are equal. So there exists $t \in T_{\alpha'}$, such that:
\[
\ad_n(e_{\pm \alpha}) = \ad_t(e_{\pm \alpha'}).
\]

Finally, using equation \ref{eq:preferred_lift}, we obtain $\Ad_n(n_\alpha) = \Ad_t(n_{\alpha'})$.
\end{proof}





\subsection{Constraints on Lie brackets}
\label{subsect:lie_bracket}

With a fixed Chevalley basis, and two roots $\alpha, \beta$, our next goal is to compute the commutator:
\begin{equation}
\label{eq:commutator_to_compute}
\exp{(-e_\beta)}\exp{(e_\alpha)}\exp{(e_\beta)}\exp{(-e_\alpha)},
\end{equation}
in terms of iterated Lie brackets of $e_\alpha$ and $e_\beta$. The result is Lemma \ref{lem:BCH}.

%\todo{BM: I have rewritten the definition of iterated Lie Bracket}
%We use the term ``iterated Lie brackets of $x$ and $y$'' to refer to all elements of $\fr g$ obtained by applying $[-,-]$ successively to finitely many copies of $x$ and $y$. In the particular case where only one copy of $y$ is used, we introduce the short-hand notation:
\begin{definition}[Iterated Lie Bracket of $x$ and $y$]
\label{def:iterated_lie}
%We iteratively define the term \emph{iterated Lie brackets of $x$ and $y$} by saying that any expression of the form $[a,b]$ where $a$ and $b$ are either an iterated Lie bracket of $x$ and $y$, or $x$, or $y$ is an iterated Lie bracket of $x$ and $y$.
We iteratively define the term \emph{iterated Lie bracket of $x$ and $y$} as any expression of the form $[a,b]$, where $a$ and $b$ are either $x$, or $y$, or an iterated Lie bracket of $x$ and $y$.
\end{definition}

We introduce the short-hand notation:
\begin{equation}
\label{eq:notation_iterated_brackets}
[x,y]^{[n]} := [x,[x,\dots [x,y]]]. 
\end{equation}  

In the case $x = e_\alpha, y = e_\beta$, we prove that all but finitely many iterated Lie brackets are 0.

\begin{lemma}
\label{lem:brackets_vanish}
Let $\alpha, \beta$ be roots of $\fr g$ such that $\alpha \neq \pm \beta$. If $\alpha$ and $\beta$ have different lengths, assume that $\alpha$ is the shorter root. Then all iterated brackets of $e_\alpha, e_\beta$ vanish, except for, at most:
\begin{equation}
\label{eq:commutator_roots}
[e_\alpha,e_\beta] \hspace{1cm} 
[e_\alpha,e_\beta]^{[2]} \hspace{1cm} 
[e_\alpha,e_\beta]^{[3]}  \hspace{1cm}
\big[[e_\alpha,e_\beta]^{[2]},[e_\alpha,e_\beta]\big]
\end{equation}
\end{lemma}

%BM: I have checked this and am now happy.

\begin{proof}
This is a statement about the structure of root systems of simple Lie algebras; see e.g. chapter 7 of \cite{kirillov_introduction} for a review of the definitions and basic properties of root systems. 

According to Lemma \ref{lem:roots_commutators_vanish}, for all roots $\gamma$ and $\delta$ with $\gamma + \delta \neq 0$, $[e_\gamma, e_\delta] = 0$ if and only if $\gamma + \delta \not \in \Phi$.
So it suffices to prove that the roots which are positive integral linear combinations of $\alpha$ and $\beta$ are, at most:
\begin{equation}
\label{eq:possible_roots}
\alpha + \beta, 
\hspace{1cm} 
2\alpha + \beta,
\hspace{1cm}
3\alpha + \beta,
\hspace{1cm}
3\alpha + 2\beta.
\end{equation}

Note first that all linear combinations of $\alpha$ and $\beta$ live in the plane determined by $\alpha$ and $\beta$, hence in a root sub-system of rank 2. Thus, it suffices to check the statement for the rank 2 root systems. There are four of them, up to equivalence; see Theorem 7.10 in \cite{kirillov_introduction} for a proof.

\begin{enumerate}
    \item In the easiest case, $A_1 \times A_1$, no positive integral linear combinations are roots. See Figure \ref{fig:a1root}.
    \begin{figure}[h]
    \centering
    \begin{minipage}{.5\textwidth}
      \centering
      \includegraphics[scale = 0.3]{Root-system-A1xA1.png}
      \caption{The root system $A_1 \times A_1$}
      \label{fig:a1root}
    \end{minipage}%
    \begin{minipage}{.5\textwidth}
      \centering
      \includegraphics[scale = 0.3]{Root-system-A2.png}
      \caption{The root system $A_2$}
      \label{fig:a2root}
    \end{minipage}
    \end{figure}
    
    \item In $A_2$, under the assumption that $\alpha \neq \pm \beta$, the magnitude of the angle between $\alpha$ and $\beta$ satisfies $\sphericalangle (\alpha, \beta) \in \{ \pi/3, 2\pi/3 \}$. In the first case, no positive integral linear combination of $\alpha$ and $\beta$ is a root. In the second case, $\alpha + \beta$ is a root, but there are no other positive integral linear combinations. See Figure \ref{fig:a2root}.

    For root systems of type ADE, the $\alpha, \beta$-plane is either of type $A_1 \times A_1$, or of type $A_2$. It follows that, in all root systems of type ADE, no positive linear combination of $\alpha$ and $\beta$ other than $\alpha + \beta$ can be a root.
    
    \item In $B_2$, $\sphericalangle (\alpha, \beta) \in \{ \pi/4, \pi/2, 3\pi/4 \}$. In the case of $3\pi/4$, both $\alpha + \beta$ and $2\alpha + \beta$ are roots. See Figure \ref{fig:b2root}.
    
    \begin{figure}[h]
    \centering
    \begin{minipage}{.5\textwidth}
      \centering
      \includegraphics[scale = 0.3]{Root-system-B2.png}
      \caption{The root system $B_2$}
      \label{fig:b2root}
    \end{minipage}%
    \begin{minipage}{.5\textwidth}
      \centering
      \includegraphics[scale = 0.3]{Root-system-G2.png}
      \caption{The root system $G_2$}
      \label{fig:g2root}
    \end{minipage}
    \end{figure}
    
    For root systems of type BCF, the $\alpha, \beta$-plane is of type $A_1 \times A_1$, $A_2$ or $B_2$. It follows that, in such root systems, at most $\alpha + \beta$ and $2\alpha + \beta$ are roots.
    
    \item In $G_2$, $\sphericalangle(\alpha,\beta) \in \{ \pi/6, \pi/3, \pi/2, 2\pi/3, 5\pi/6\}$. In the case of $5 \pi/6$, all possibilities listed in \ref{eq:possible_roots} are realized. See Figure \ref{fig:g2root}.
      
\end{enumerate}
\end{proof}


As a preliminary step to computing the commutators \ref{eq:commutator_to_compute}, we prove two lemmas that make sense only for $G = GL(n)$. They make use of the associative algebra structure on $\fr g = \fr{gl}_n$, of which the Lie bracket is the commutator. 

\begin{lemma}
\label{lem:conj_exp}
Let $G = GL(n)$, and $x,y \in \fr{gl}_n$. Then:
\[   e^x e^y e^{-x} = e^y + \sum_{n=1}^\infty \frac{[x,e^y]^{[n]}}{n!}.   \]
\end{lemma}
\begin{proof}
%\todo{MI edited this proof 1/17; check}  BM Checked -- I made a clarification of what exponential map you were taking.
The claim is the specialization to $t=1$ of:
\[
e^{tx} e^y e^{-tx} = \exp(\ad_{tx}) e^y,
\]
where by we are taking the exponential map $exp: \mathfrak{gl}(\fg)\rightarrow GL(\mathfrak{g})$.

To prove the latter, let $f(t)$ denote the LHS. Then $f(0) = e^y$, and:
\[
\frac{df}{dt} = x e^{tx} e^y e^{-tx} - e^{tx} e^y e^{-tx} x = \ad_{x} f(t) .
\]
Then:
\[
f(t) = e^{\ad_{tx}} f(0) = \exp(\ad_{tx}) e^y.
\]
\end{proof}

\begin{lemma}
\label{lem:comm_exp}
Let $G = GL(n)$, and $x,y\in \fr{gl}_n$. Then:
\[
[x,e^y] = \int_0^1 e^{(1-s) y} [x,y] e^{sy} ds .
\]
If, moreover, $\big[y, [x,y] \big] = 0$, this reduces to:
\[
[x, e^y] = [x,y] e^y.
\]
\begin{proof}
The first statement follows from a straightforward computation that the authors found at \cite{stackex-exp}.
It is the $t=1$ specialization of:
\[   e^{-ty} [x,e^{ty}] = \int_0^t e^{-s y} [x,y] e^{s y} ds .   \]
This identity is true at $t=0$, and both sides have the same first derivative as a function of $t$.

For the second statement, under the assumption that $\big[y, [x,y] \big] = 0$ the integrand becomes:
\[
e^{(1-s)y} [x,y] e^{sy} = [x,y] e^{(1-s)y} e^{sy} = [x,y] e^y.
\]
\end{proof}
\end{lemma}



Finally, using the previous lemmas, we compute the commutator \ref{eq:commutator_to_compute}.

\begin{lemma}
\label{lem:BCH}
Let $G$ be a connected reductive algebraic group over $\C$. Let $x, y \in \fr{g}$ such that all their iterated Lie brackets vanish, except, at most, for the following:
\[
[x,y] 
\hspace{1cm} 
[x,y]^{[2]} := [x,[x,y]] 
\hspace{1cm} 
[x,y]^{[3]} := \big[x,[x,[x,y]]\big]
\hspace{1cm}
\big[[x,y]^{[2]},[x,y]\big] .
\]
(By Lemma \ref{lem:brackets_vanish}, this covers the case $x = e_\alpha$, $y = e_\beta$ in which we are interested.)
Then the following holds in $G$:
\begin{equation}
\label{eq:ugly_formula}
e^{-y} e^x e^y e^{-x}
= 
\exp{[x,y]}
\exp\left(\frac{1}{6} \big[[x,y]^{[2]},[x,y]\big]\right)
\exp\left(\frac{1}{2} [x,y]^{[2]}\right) 
\exp\left(\frac{1}{6} [x,y]^{[3]}\right)
\end{equation}
\end{lemma}

% Proof approved by BM January 23rd

\begin{proof}
Choose any faithful, finite dimensional representation $\rho : G \to GL(n)$. Because $\rho$ preserves the relation \ref{eq:ugly_formula}, it suffices to prove the claim for $GL(n)$.

Multiplying the result of Lemma \ref{lem:conj_exp} on the left by $e^{-y}$ we obtain:
\[      
e^{-y}e^x e^y e^{-x} 
= 
\id + 
\sum_{n=1}^\infty 
e^{-y} \frac{[x,e^y]^{[n]}}{n!}  .
\]
So it suffices to prove that:
\begin{equation}
\label{eq:two_expansions}
\id + 
\sum_{n=1}^\infty 
\frac{[x,e^y]^{[n]}}{n!} e^{-y}
=
\exp{[x,y]}
\exp\left(\frac{1}{6} \big[[x,y]^{[2]},[x,y]\big]\right)
\exp\left(\frac{1}{2} [x,y]^{[2]}\right) 
\exp\left(\frac{1}{6} [x,y]^{[3]}\right)
.
\end{equation}

The strategy is to expand both the LHS and the RHS of \ref{eq:two_expansions} as sums of terms of the form:
\[
T_{n,i,j,k} 
= 
([x,y])^{n-3i-2j-3k}
(\big[[x,y]^{[2]},[x,y]\big])^i
([x,y]^{[2]})^j
([x,y]^{[3]})^k 
.
\]
Note that $n$ is the $x$-degree of $T_{n,i,j,k}$. The expansions we look for are:
%\todo{make a comment about uniqueness}
\begin{align*}
LHS
&=
\sum_{n,i,j,k} a_{n,i,j,k}  T_{n,i,j,k},
\\
RHS
&=
\sum_{n,i,j,k} b_{n,i,j,k}  T_{n,i,j,k} .
\end{align*}


%\todo{Benedict: I completely rewrote the text, as what you wrote was deeply confusing, and probably wrong.}
For the left hand side we will write get an expression of the above form by for each $n$ writing $e^{-y}\frac{[x,e^{y}]^{[n]}}{n!}=\sum_{i,j,k}a_{n,i,j,k}T_{n,i,j,k}$ (where we consider the term corresponding to $n=0$ to be $Id$).  We then have.  
%All exponents appearing in $T_{n,i,j,k}$ must be non-negative \todo{Why?  Isn't it rather that you're making a choice such that this is the case.}, so $a_{n,i,j,k} = b_{n,i,j,k} = 0$ unless $i,j,k \geq 0$ and $3i + 2j + 3k \leq n$.
%The goal is to prove that $a_{n,i,j,k} = b_{n,i,j,k}$.

%To obtain the expansion of the LHS, note that for a fixed $n$, all terms with $x$-degree equal to $n$ come from $e^{-y} [x,e^y]^{[n]}$ \todo{No -- this is not clear again because uniqueness is clear -- rather say that we get an equation of the form $LHS=\sum$ by writing $[x, e^{y}]^[n]=\sum_{i,j,k}a_{n,i,j,k}T_{n,i,j,k}$}. We see that:
\begin{enumerate}
    \item If $n=0$, then $Id=T_{0,0,0,0}$ so we set $a_{0,0,0,0} = 1$, and all other $a_{0,i,j,k} = 0$.
    \item If $n=1$, Lemma \ref{lem:comm_exp} and the fact that $[y,[x,y]] = 0$ imply that:
    \begin{equation}
    \label{eq:n=1_commutator}
    e^{-y} [x,e^y] 
    = 
    e^{-y} [x,y] e^y = [x,y] .
    \end{equation}
    So we set $a_{1,0,0,0} = 1$, and all other $a_{1,i,j,k} = 0$.
    \item For $n>1$, we can inductively obtain an expression for $[x,e^y]^{[n+1]}$ by applying $[x,-]$ to the current expression for $[x,e^y]^{[n]}$:
    \[
    \frac{[x,e^y]^{[n]}}{n!} 
    = 
    \sum_{i,j,k} 
    a_{n,i,j,k} e^{y} T_{n,i,j,k} .
    \]
    We repeatedly use the product rule $[x, ab] = [x,a] b + a [x,b]$ to reduce the computation of the bracket $\big[x, e^y T_{n,i,j,k} \big]$ to the computations:
    \begin{align*}
    \big[ x, e^y \big] &= e^y [x,y],
    \\
    \big[ x, ([x,y])^l ] &= l ([x,y])^{l-1} [x,y]^{[2]} + \frac{l(l-1)}{2} ([x,y])^{l-2} \big[[x,y]^{[2]},[x,y] \big],
    \\
    \Big[ x, \big(\big[[x,y]^{[2]},[x,y] \big]\big)^i \Big] &= 0,
    \\
    \big[ x, ([x,y]^{[2]})^j \big] &= j ([x,y]^{[2]})^{j-1} [x,y]^{[3]},
    \\
    \big[ x, ([x,y]^{[3]})^k \big] &= 0.
    \end{align*}
    In deriving the relations above, we used the product rule inductively, and used commutators to permute factors past each other. Most of the factors involved actually commute, due to the hypothesis of the current lemma.
    Putting all these terms together, with $l = n - 3i - 2j - 3k$, yields:
    \begin{align*}
    \frac{[x,e^y]^{[n+1]}}{(n+1)!}
    =
    \sum_{i,j,k}
    \frac{a_{n,i,j,k}}{n+1} e^{y}
    &
    \bigg(
    T_{n+1,i,j,k} + j T_{n+1,i,j-1,k+1}
    +
    (n-3i-2j-3k) T_{n+1,i,j+1,k}
    \\
    &+
    \frac{(n-3i-2j-3k)(n-3i-2j-3k-1)}{2} 
    T_{n+1,i+1,j,k}.
    \bigg)
    \end{align*}
    
    From here we can read off a recurrence relation for the coefficients:
    \begin{align}
    \begin{split}
    \label{eq:BCH_recursion}
    (n+1) a_{n+1,i,j,k} 
    =& 
    a_{n,i,j,k} + (j+1) a_{n,i,j+1,k-1} 
    \\
    &+
    \big(n-3i-2(j-1)-3k\big) a_{n,i,j-1,k} 
    \\
    &+
    \frac{\big(n-3(i-1)-2j-3k \big)\big(n-3(i-1)-2j-3k -1 \big)}{2} a_{n,i-1,j,k} .
    \end{split}
    \end{align}
    
    This relation determines uniquely the coefficient $a_{n,i,j,k}$, in terms of coefficients $a_{n',i',j',k'}$ with $n' < n$. So the recurrence relation has a unique solution, once we specify the initial condition $a_{0,0,0,0} = 1$.
\end{enumerate}


We now carry out the expansion:
\[
RHS
=
\sum_{n,i,j,k} b_{n,i,j,k}  T_{n,i,j,k},
\]
by taking the Taylor series of the exponentials in RHS. We obtain closed form expressions for $b_{n,i,j,k}$:
\[
b_{n,i,j,k}
=
\frac{1}{(n-3i-2j-3k)!}
\frac{1}{6^i i!}
\frac{1}{2^j j!}
\frac{1}{6^k k!}.
\]
By direct verification, $b_{n,i,j,k}$ solve the recurrence relation \ref{eq:BCH_recursion}, with the same initial condition $b_{0,0,0,0} = 1$. Therefore $b_{n,i,j,k} = a_{n,i,j,k}$ for all $n,i,j,k$.
\end{proof}





\subsection{Stokes Data}
\label{sec: Stokes Data}

In non-abelianization we are going to be modifying a given $G$-bundle by unipotent automorphisms along a set of geodesics on $X$.  As already noted when these geodesics intersect we may need to add additional geodesics, as well as assigning these unipotent automorphisms (as in the Cecotti--Vafa wall crossing formula).  We do this in this section.

Consider an intersection of Stokes rays labelled by the roots $\alpha_{1},\alpha_{2},...,\alpha_{j}$ of a Lie algebra $\fg$, with root system $\Phi\subset \ft^{*}$.

\begin{definition}[Cone of a set of roots]
\label{def:cone_roots}
The \emph{Cone} of a set of roots $\alpha_{1},...,\alpha_{j}$ is the set $C_{\alpha_{1},...,\alpha_{j}}:=\Sigma_{i=1}^{j}\bbR_{\geq 0}\alpha_{i}\subset \ft^{*}$.
\end{definition}

We will restrict to the case where the set of roots is convex in the following sense:

\begin{definition}[Convex set of roots]
\label{def: convex set of roots}
  We say that a set of roots is \emph{convex} if the cone $C_{\alpha_{1},...,\alpha_{j}}\subset \ft^{*}$ is strongly convex, in that it does not contain a 1d real vector space.
\end{definition}

\begin{definition}
%[Nilpotent Lie algebra associated to a polyhedron]
\label{definition: poyhedral nilpotent lie algebra}
We define the following Lie algebras:
\begin{itemize}
    \item For $\alpha \in \Phi$, let $\fu_\alpha$ denote the root space $\fg_\alpha$.
    \item For $\{\alpha_1, \dots, \alpha_j\}$ a convex set of roots define the Lie algebra generated by $\fu_{\alpha_1}, \dots, \fu_{\alpha_n}$:
    \[
    \fu_{\alpha_1, \dots, \alpha_n}
    :=
    \langle \fu_{\alpha_1} , \dots, \fu_{\alpha_n} \rangle .
    \]
    \item Given a strongly convex rational (with respect to the weight lattice) polyhedron $\Delta\subset \ft^{*}$, we define the associated Lie algebra:
    \[
    \fu_{\Delta}
    :=
    \bigoplus_{\gamma \in \Phi\cap\Delta}\fu_{\gamma}.
    \]
\end{itemize}
\end{definition}

Henceforth when we refer to a cone in $\ft^{*}$ we refer to a strongly convex cone, which is rational with respect to the weight lattice.

\begin{lemma}
For $\{\alpha_1, \dots, \alpha_j\}$ a convex set of roots, there is an inclusion of Lie algebras:
\[
\fu_{\alpha_1, \dots, \alpha_j}
\hookrightarrow
\fu_{C_{\alpha_{1}, \dots ,\alpha_{j}}}.
\]
\end{lemma}

\begin{proof}
A basis for $\fu_{\alpha_1, \dots, \alpha_j}$ is given by iterated Lie brackets of $e_{\alpha_1}, \dots, e_{\alpha_j}$, in the sense of Definition \ref{def:iterated_lie}.
Recall the result of Lemma \ref{lem:roots_commutators_vanish}, which says that for all $\beta, \gamma \in \Phi$, $[\fg_\beta, \fg_\gamma] \subset \fg_{\beta + \gamma}$. 
By recursive application of this result, we obtain that all iterated Lie brackets of $e_{\alpha_1}, \dots, e_{\alpha_j}$ are in the root spaces of roots contained in the cone of $\{\alpha_{1},\alpha_{2},...,\alpha_{j}\}$.
\end{proof}

\begin{lemma}
All Lie algebras from Definition \ref{definition: poyhedral nilpotent lie algebra} are nilpotent.
\end{lemma}

\begin{proof}
Due to the convexity assumption, there exists a polarization $\Phi = \Phi_+ \coprod \Phi_-$ of the root system, such that $\{\alpha_1, \dots, \alpha_j\} \subset \Phi_+$. Recall that the Lie algebra:
\[
\fr{n}_+ = \bigoplus_{\alpha \in \Phi_+} \fg_\alpha
\]
is nilpotent. 
%This fact is standard. \todo{find reference} Its proof uses the Serre relations $(\ad e_{\alpha_i})^{1-a_{ij}} e_{\alpha_j} = 0$, for all $\alpha_i, \alpha_j \in \Phi_+$, which show that the operators $\ad e_{\alpha_i}$ acting on $\fr n_+$ are nilpotent, with order of nilpotency $\max_j \{1-a_{ij}\}$. Furthermore, Engel's theorem ensures that nilpotency of $\ad e_{\alpha}$ for all $\alpha \in \Phi_+$ is equivalent to nilpotency of $\fr{n}_+$.
The Lie algebras in Definition \ref{definition: poyhedral nilpotent lie algebra} are Lie subalgebras of $\fr n_+$. Lie subalgebras of nilpotent Lie algebras are nilpotent.
\end{proof}

\begin{definition}
For any strongly convex rational polyhedron $\Delta$, let $U_\Delta := \exp (\fu_\Delta)$ be the corresponding unipotent group. Similarly, for any set of convex roots $\{\gamma_1, \dots, \gamma_k\}$, let $U_{\gamma_1, \dots, \gamma_k} := \exp ( \fu_{\gamma_1, \dots, \gamma_k})$.
\end{definition}

\begin{remark}
Note that, for any nilpotent Lie algebra $\fu$, the exponential map $\exp : \fu \to U$ is algebraic. (The Taylor series is finite.) Therefore, all constructions in this section that involve the exponential map makes sense in the setting of algebraic groups.
\end{remark}




\begin{definition}
\label{def:convex_hulls}
Let $\{\alpha_1, \dots, \alpha_j\}$ be a convex set of roots. Their \textbf{convex hull} is:
\[
\Conv_{\alpha_1, \dots, \alpha_j}
:=
\Phi \cap C_{\alpha_{1},...,\alpha_{j}}.
\]
Their \textbf{restricted convex hull} is the subset of the convex hull consisting of elements which are non-negative integral linear combinations:
\[
\Conv^\N_{\alpha_1, \dots, \alpha_j} 
:=
\left\{ 
\gamma \in \Conv_{\alpha_1, \dots, \alpha_j} 
| 
\gamma = \sum_{i=1}^j n_i \alpha_i, 
\; 
n_i \in \N 
\right\} .
\]

Given two roots $\alpha_1 \neq \pm \alpha_2$, $\Conv_{\alpha_1, \alpha_2}$ (and $\Conv^\N_{\alpha_1, \alpha_2}$) is a planar, convex set of roots. We define the \textbf{planar order} as the total order on elements $\gamma \in \Conv_{\alpha_1, \alpha_2}$ (or $\Conv^\N_{\alpha_1, \alpha_2}$) induced by the magnitude of the angle $\sphericalangle (\gamma,\alpha_1)$. For example, $\alpha_1$ is the smallest element, and $\alpha_2$ is the largest.
\end{definition}

The restricted convex hull is motivated by the following reinterpretation of Lemma \ref{lem:BCH}. For $S$ a totally ordered index set, we use the notation $\overrightarrow{\prod}_{s \in S}$ or $\overleftarrow{\prod}_{s \in S}$
to refer to the product in which factors appear in increasing or decreasing order of their index, respectively.

\begin{lemma}
\label{lem:ugly_formula_interpretation}
Let $\{\alpha_1, \alpha_2\}$ be a convex set of roots. Arrange the elements $\gamma \in \Conv^\N_{\alpha_1, \alpha_2}$ in the planar order, introduced in Definition \ref{def:convex_hulls}. Then there is a morphism $\phi$ of schemes, which commutes with the multiplication maps:
\[
\begin{tikzcd}
U_{\alpha_2} \times U_{\alpha_1} 
\arrow{r}{m}
\arrow[swap]{d}{\phi }
&
G
\\
\overrightarrow{\prod}_{\gamma \in \Conv^\N_{\alpha_1,\alpha_2}} U_{\gamma}
\arrow[swap]{ur}{m}
&
\end{tikzcd}
\]
\end{lemma}

\begin{proof}
This is just a reformulation of Lemma \ref{lem:BCH}; $\phi$ is obtained from:
\begin{align*}
U_{\alpha_2} \times U_{\alpha_1} 
&\longrightarrow
\overrightarrow{\prod}_{\gamma \in \Conv^\N_{\alpha_1,\alpha_2}} U_{\gamma} 
\\
(e^y, e^x) 
&\longmapsto
\Bigg(e^y,
\exp{[x,y]},
\exp\left(\frac{1}{6} \big[[x,y]^{[2]},[x,y]\big]\right),
\exp\left(\frac{1}{2} [x,y]^{[2]}\right),
\exp\left(\frac{1}{6} [x,y]^{[3]}\right),
e^x
\Bigg),
\end{align*}
by skipping an element if the bracket in the exponent is zero.
\end{proof}

\begin{example}
In a root system of type B2 (see Figure \ref{fig:b2root}), let $\alpha_1, \alpha_2$ be orthogonal long roots. Then:
\begin{align*}
\Conv_{\alpha_1, \alpha_2} &= \{\alpha_1, (\alpha_1 + \alpha_2)/2, \alpha_2\},
\\
\Conv^\N_{\alpha_1, \alpha_2} &= \{\alpha_1,  \alpha_2\}.
\end{align*}
In this case, multiplication between $U_{\alpha_1}$ and $U_{\alpha_2}$ in $G$ is commutative, so the morphism $\phi$ from Lemma \ref{lem:ugly_formula_interpretation} is the transposition $U_{\alpha_2} \times U_{\alpha_1} \to U_{\alpha_1} \times U_{\alpha_2}$.
\end{example}

\begin{example}
In root systems of type ADE, for every convex pair $\{\alpha_1, \alpha_2\}$, $\Conv_{\alpha_1, \alpha_2} = \Conv^\N_{\alpha_1, \alpha_2}$. To see this, note that the restriction of the root system to the plane spanned by $\alpha_1$ and $\alpha_2$ is a root system of type $A_1 \times A_1$ or $A_2$. In both cases, the claim is obvious. (See Figures \ref{fig:a1root} and \ref{fig:a2root}.)
\end{example}

The following result is a generalization of Lemma \ref{lem:ugly_formula_interpretation}; it will be used to assign Stokes factors to new Stokes curves in Lemma \ref{lem:assignment_stokes_newlines_equivariant}.

\begin{proposition}
\label{prop: Ultimately uniqueness of Stokes data}
Let $\alpha_1 \neq \alpha_2$ be two roots, and $\{\gamma_1, \dots, \gamma_n\} = \Conv^\N_{\alpha_1,\alpha_2}$, where the order is arbitrary.
Multiplication gives an isomorphism of schemes:
\[
U_{\gamma_{1}}\times ...\times U_{\gamma_{n}}\xrightarrow{\cong} U_{\Conv^\N_{\alpha_1,\alpha_2}} .
\]
Moreover, this isomorphism is equivariant with respect to the adjoint action of $N$, acting diagonally on the LHS. Therefore it descends to an isomorphism of stacks:
\[
\left(
\coprod U_{\gamma_{1}}\times ...\times U_{\gamma_{n}}
\right)
/N
\xrightarrow{\cong}
\left(
\coprod U_{\Conv^\N_{\alpha_1,\alpha_2}}
\right) / N,
\]
where the disjoint union is over the orbits of the diagonal $W$ action.
\end{proposition}

Before giving the proof of this proposition, we first state and prove Lemmas \ref{lem:iso_generated} - \ref{lem:mult_surjective}.

\begin{lemma}
\label{lem:iso_generated}
There is an isomorphism of Lie groups:
\[
\langle U_{\gamma_{1}},...,U_{\gamma_{n}} \rangle \xrightarrow{\cong}U_{\Conv^\N_{\alpha_1,\alpha_2}},
\]
where the left hand side is the subgroup  of $G$ generated by $U_{\gamma_{1}},\dots, U_{\gamma_{n}}$.  
\end{lemma}

\begin{proof}
As $U_{\gamma_{i}}\subset U_{\Conv^\N_{\alpha_1,\alpha_2}}$ for each $1\leq i\leq n$, it is clear that multiplication gives us such a map; denote it by $mult$.
The map $mult$ induces an isomorphism on Lie algebras, by definition \ref{definition: poyhedral nilpotent lie algebra} and Lemma \ref{lem:roots_commutators_vanish}. Moreover, both Lie algebras are nilpotent, so the exponential maps in the following commutative diagram are isomorphisms:
\[
\begin{tikzcd}
\langle U_{\gamma_{1}},...,U_{\gamma_{n}} \rangle
\arrow{r}{mult}
&
U_{\Conv^\N_{\alpha_1,\alpha_2}}
\\
\langle \fu_{\gamma_{1}},...,\fu_{\gamma_{n}} \rangle
\arrow{r}{\cong}
\arrow{u}{\exp }
&
\fu_{\Conv^\N_{\alpha_1,\alpha_2}}
\arrow[swap]{u}{\exp}
\end{tikzcd}
\]
It follows that $mult$ is the composition of three isomorphisms, hence a isomorphisms. Moreover, $mult$ is a group homomorphism. So it's an isomorphism of Lie groups.
\end{proof}


\begin{lemma}
\label{lem:sort_sigma}
Let $\sigma \in S_n$ be any permutation. Then, in the setting of Proposition \ref{prop: Ultimately uniqueness of Stokes data}, there exists an isomorphism of schemes $\sort_\sigma$, which commutes with the multiplication maps:
\begin{equation}
\label{diag:sort_map}
\begin{tikzcd}
U_{\gamma_{1}}\times \dots \times U_{\gamma_{n}}
\arrow{r}{m} \arrow[swap]{d}{\sort_\sigma}
&
U_{\Conv^\N_{\alpha_1,\alpha_2}}
\\
U_{\gamma_{\sigma(1)}}\times \dots \times U_{\gamma_{\sigma(n)}}
\arrow[swap]{ur}{m'}
\end{tikzcd}
\end{equation}
\end{lemma}

\begin{proof}
%Assume that $\gamma_1, \dots, \gamma_n$ are coplanar. Because of this, there is a total order $<$ on the set $\{\gamma_i\}_{i=1}^n$, satisfying the following condition. For all $i,j$ such that $\gamma_i < \gamma_j$, and all $k$ such that $\gamma_k$ is in the interior of the cone $C_{\gamma_i, \gamma_j}$, we have:
%\begin{equation}
%label{eq:total_order_roots}
%\gamma_i < \gamma_k < \gamma_j
%\end{equation}
%\todo{picture necessary?}

It suffices to construct $\sort_\sigma$ in the case that the output of $\sigma$ is ordered increasingly with respect to the planar order of Definition \ref{def:convex_hulls}, i.e.:
\begin{equation}
\label{eq:sigma_sorting}
\gamma_{\sigma(1)} < \dots < \gamma_{\sigma(n)}.
\end{equation}
Having dealt with this case, we can then define $\sort_{\sigma^{-1}} = (\sort_\sigma)^{-1}$. Moreover, for any other permutation $\tau \in S_n$, we can decompose it as $(\tau \circ \sigma^{-1}) \circ \sigma$, so that we have:
\[
\begin{tikzcd}
\{1, \dots, n\}
\arrow[mapsto]{r}{\sigma} 
&
\{\sigma(1), \dots, \sigma(n) \}
\arrow[mapsto]{r}{\tau \circ \sigma^{-1}}
&
\{\tau(1), \dots, \tau(n)\}
\end{tikzcd}
\]
and the outputs of both $(\tau \circ \sigma^{-1})^{-1}$ and $\sigma$ satisfy \ref{eq:sigma_sorting}. Then we define $\sort_\tau$ as the composition:
\[
\begin{tikzcd}
U_{\gamma_1} \times \dots \times U_{\gamma_n} 
\arrow{r}{\sort_\sigma} 
&
U_{\gamma_{\sigma(1)}} \times \dots \times U_{\gamma_{\sigma(n)}}
\arrow{r}{\sort_{\tau\circ \sigma^{-1}}}
&
U_{\gamma_{\tau(1)}} \times \dots \times U_{\gamma_{\tau(n)}}
\end{tikzcd}
\]
In doing this, because $\sort_\sigma$ and $\sort_{\tau \sigma^{-1}}$ are isomorphisms, so is $\sort_\tau$.

Let $\sigma \in S_n$ be the unique permutation such that \ref{eq:sigma_sorting} holds. We define $\sort_\sigma$ as a composition of twisted transpositions and contractions.\footnote{$\sort_\sigma$ is similar to the ``bubble sort'' algorithm; the difference are the new factors which appear due to non-commutativity of group elements.}
Concretely, say that $\gamma_i > \gamma_j$; a twisted transposition is a map:
\begin{equation}
\label{eq:transposition}
U_{\gamma_i} \times U_{\gamma_j}
\to 
\overrightarrow{\prod_{\gamma_k \in \Conv^\N_{\gamma_j,\gamma_i}}} U_{\gamma_k} .
\end{equation}
as described in Lemma \ref{lem:ugly_formula_interpretation}.
It sends an element $(e^x, e^y) \in U_{\gamma_i} \times U_{\gamma_j}$ to the tuple:
\[
\Bigg(e^y,
\exp{[x,y]},
\exp\left(\frac{1}{6} \big[[x,y]^{[2]},[x,y]\big]\right),
\exp\left(\frac{1}{2} [x,y]^{[2]}\right),
\exp\left(\frac{1}{6} [x,y]^{[3]}\right),
e^x
\Bigg),
\]
where the tuple is sorted increasingly with respect to the planar order of Definition \ref{def:convex_hulls}.
Equation \ref{eq:ugly_formula} ensures that the product $e^x e^y$, evaluated in $G$, is equal to the ordered product of all elements in the tuple.

A contraction is a multiplication map:
\begin{align*}
U_{\gamma_i} \times U_{\gamma_i} &\to U_{\gamma_i}
\\
(u_1, u_2) &\mapsto u_1u_2 .
\end{align*}
    
We define $\sort_\sigma$ as follows. Start with the factor $U_{\gamma_{\sigma(1)}}$, and apply twisted transpositions to move it left past other factors, until it is on the leftmost position. Then do the same with all occurrences of $U_{\gamma_{\sigma(2)}}$, and so on. Contract neighboring instances of the same factor $U_{\gamma_i}$ whenever they occur. Examples of this procedure can be seen in equations \ref{eq:sort_A2} - \ref{sort_G2} below.
    
To show that $\sort_\sigma$ is an isomorphism, note that $\Conv^\N_{\alpha_1,\alpha_2}$ are contained in a planar root system. There are four such root systems (see Figures \ref{fig:a1root} - \ref{fig:g2root}); we treat the cases separately. In all cases, for $i<j$, introduce a constant $c_{ij}$ which is equal to 0 if $\sigma(1) < \sigma(3)$, and 1 otherwise.
    
\begin{enumerate}
    \item For $A_1 \times A_1$, the largest cardinality of a convex set of roots is 2. In this case, $U_1$ and $U_2$ commute, and $\sort_\sigma$ is the honest permutation $U_1 \times U_2 \to U_{\sigma(1)} \times U_{\sigma(2)}$, which is invertible.
    
    \item For $A_2$, the largest cardinality of a convex set of roots is 3. If $\sigma(1) < \sigma(3)$, then $\sort_\sigma$ is an honest permutation. Otherwise, since multiplication between $U_{\sigma(1)}$ and $U_{\sigma(3)}$ is non-commutative, we need a twisted transposition to commute $U_{\sigma(1)}$ past $U_{\sigma(3)}$. 
    %To treat both cases simultaneously, introduce a constant $c_{13}$, which is equal to 0 if $\sigma(1) < \sigma(3)$, and 1 otherwise. 
    Then $\sort_\sigma$ is the map:
\begin{equation}
\label{eq:sort_A2}
\begin{tikzcd}
\big( \exp(X_1) , \exp(X_2) ,
\exp(X_3) \big)
\arrow[mapsto]{d}
\\
\Big( 
\exp\big(X_{\sigma(1)}\big),
\exp\big(X_{\sigma(2)} + c_{13} [X_{\sigma(3)},X_{\sigma(1)}]\big),
\exp\big(X_{\sigma(3)}\big)
\Big).
\end{tikzcd}
\end{equation}
This is invertible: given the output, we can recover first $X_{\sigma(1)}$ and $X_{\sigma(3)}$, then $X_{\sigma(2)}$.

\item For $B_2$, the largest cardinality of a convex set of roots is 4. With labels as in Figure \ref{fig:B2_convex}, $\sort_\sigma$ is the map:
\begin{equation}
\label{sort_B2}
\begin{tikzcd}
\big( \exp(X_1) , \exp(X_2) ,\exp(X_3), \exp(X_4) \big)
\arrow[mapsto]{d}
\\
\Big(
\exp\big(X'_{\sigma(1)}\big), 
\exp\big(X'_{\sigma(2)}\big), 
\exp\big(X'_{\sigma(3)}\big), 
\exp\big(X'_{\sigma(4)}\big)
\Big),
\end{tikzcd}
\end{equation}
where:
\begin{align*}
X'_{\sigma(1)} &= X_{\sigma(1)}
\\
X'_{\sigma(2)} &= X_{\sigma(2)}
+ c_{14} [X_{\sigma(4)},X_{\sigma(1)}]
\\
X'_{\sigma(3)} &= X_{\sigma(3)}
+ c_{24} [X_{\sigma(4)},X_{\sigma(2)}] + \frac{1}{2} c_{14}[X_{\sigma(4)},X_{\sigma(1)}]^{[2]}
\\
X'_{\sigma(4)} &= X_{\sigma(4)}
\end{align*}
This is invertible, because given the output, we can recover $X_{\sigma(1)}$, $X_{\sigma(4)}$, $X_{\sigma(2)}$, $X_{\sigma(3)}$ in this order.


\begin{figure}[h]
    \centering
    \begin{minipage}{.5\textwidth}
      \centering
      \includegraphics[scale = 0.5]{images/B2_convex.png}
      \caption{A maximal convex set of roots for B2.}
      \label{fig:B2_convex}
    \end{minipage}%
    \begin{minipage}{.5\textwidth}
      \centering
      \includegraphics[scale = 0.5]{images/G2_convex.png}
      \caption{A maximal convex set of roots for G2.}
      \label{fig:G2_convex}
    \end{minipage}
\end{figure}


\item For G2, the largest cardinality of a convex set of roots is 6. 
 With labels as in Figure \ref{fig:G2_convex}, $\sort_\sigma$ is:
\begin{equation}
\label{sort_G2}
\begin{tikzcd}
\big( \exp(X_1) , \exp(X_2) ,\exp(X_3), \exp(X_4), \exp(X_5), \exp(X_6) \big)
\arrow[mapsto]{d}
\\
\Big(
\exp\big(X'_{\sigma(1)}\big), 
\exp\big(X'_{\sigma(2)}\big), 
\exp\big(X'_{\sigma(3)}\big), 
\exp\big(X'_{\sigma(4)}\big),
\exp\big(X'_{\sigma(5)}\big),
\exp\big(X'_{\sigma(6)}\big)
\Big),
\end{tikzcd}
\end{equation}
where:
\begin{align*}
X'_{\sigma(1)} =& X_{\sigma(1)}
,
\\
X'_{\sigma(2)}
=& 
X_{\sigma(2)} + c_{16} [X_{\sigma(6)},X_{\sigma(1)}]
, 
\\
X'_{\sigma(3)} 
=& 
X_{\sigma(3)} 
+ c_{24} [X_{\sigma(4)},X_{\sigma(2)}] 
+ c_{15} [X_{\sigma(5)},X_{\sigma(1)}]
\\
&
+ \frac{1}{2} c_{12} c_{16}\big[[X_{\sigma(6)},X_{\sigma(1)}]^{[2]},X_{\sigma(2)}\big] 
\\
&
+ \frac{1}{6}c_{16} \big[[X_{\sigma(6)},X_{\sigma(1)}], [X_{\sigma(6)}, X_{\sigma(1)}]^{(2)}\big]
, 
\\
X'_{\sigma(4)} 
=&
X_{\sigma(4)} 
+ c_{26}[X_{\sigma(6)},X_{\sigma(2)}]
+ \frac{1}{2} c_{16}[X_{\sigma(6)}, X_{\sigma(1)}]^{[2]}
,
\\
X'_{\sigma(5)} 
=&
X_{\sigma(5)} + c_{46} [X_{\sigma(6)},X_{\sigma(4)}] + c_{16} \frac{1}{6} [X_{\sigma(6)},X_{\sigma(1)}]^{(3)}
,
\\
X'_{\sigma(6)} =& X_{\sigma(6)}.
\end{align*}
This is invertible, because given the output, we can recover $X_{\sigma(1)}$, $X_{\sigma(6)}$, $X_{\sigma(2)}$, $X_{\sigma(4)}$, $X_{\sigma(5)}$, $X_{\sigma(3)}$ in this order.
\end{enumerate}
\end{proof}


\begin{lemma}
\label{lem:mult_surjective}
In the setting of Proposition \ref{prop: Ultimately uniqueness of Stokes data}, the morphism:
\[
U_{\gamma_{1}}\times \dots \times U_{\gamma_{n}}
\overset{m}{\rightarrow} 
\langle U_{\Conv^\N_{\alpha_1,\alpha_2}} \rangle
\]
given by multiplication in $G$ is an isomorphism of schemes.
\end{lemma}

\begin{proof}
By Lemma \ref{lem:sort_sigma}, it suffices to prove this in the case that $\gamma_1 < \dots < \gamma_n$,
using the planar order from Definition \ref{def:convex_hulls}. Indeed, if the roots are not ordered in this way, we let $\sigma \in S_n$ be the permutation which orders the roots, and we compose $m$ with the isomorphism $\sort_\sigma$ to obtain the result.

Under the assumption that $\gamma_1 < \dots < \gamma_n$, we first prove that $m$ is surjective.
Any element $u \in U_{\Conv^\N_{\alpha_1,\alpha_2}}$ is a word in elements of $U_{\gamma_1}, \dots, U_{\gamma_n}$. 
Using twisted transpositions and contractions, just like in the construction of $\sort_\sigma$ in the proof of Lemma \ref{lem:sort_sigma}, we can commute all occurrences of elements of $U_{\gamma_1}$ to the left, then continue with all occurrences of elements of $U_{\gamma_2}$, and so on. We obtain a tuple $(u_1, \dots, u_n) \in U_{\gamma_1} \times \dots \times U_{\gamma_n}$, such that $m(u_1, \dots, u_n) = u$.

Next, we prove that $m$ is injective. Assume that there are two tuples $(u_1, \dots, u_n)$ and $(u_1', \dots, u_n') \in U_{\gamma_1} \times \dots \times U_{\gamma_n}$ such that:
\[
u_1 \dots u_n = u_1' \dots u_n' .
\]
Then:
\[
{u_1'}^{-1}u_1 = (u_2' \dots u_n')(u_2 \dots u_{n})^{-1} .
\]
Notice that the LHS is an element of $U_{\gamma_1}$, while the RHS is an element of $U_{\gamma_2, \dots, \gamma_n}$.\footnote{Here we use the fact that the set $\{ \gamma_2, \dots, \gamma_n\}$ is convex, which follows from the ordering assumption made in the first paragraph.}
Since $U_{\gamma_1} \cap U_{\gamma_2, \dots, \gamma_n} = \{\id\}$, it must be the case that $u_1 = u_1'$. By an inductive argument, it follows that $(u_1, \dots, u_n) = (u_1', \dots, u_n')$.

Hence $m$ is an isomorphism.
\end{proof}

\begin{proof}[Proof of Proposition \ref{prop: Ultimately uniqueness of Stokes data}]
Note that this map is the composition of the isomorphisms in the above two lemmas, hence it's an isomorphism.

The equivariance statement follows immediately: if we apply the diagonal adjoint action of $N$ on the LHS and multiply, we obtain:
\begin{align*}
m\big( \Ad_n(u_1) , \dots, \Ad_n(u_n) \big)
&= \Ad_n\big( m(u_1, \dots, u_n) \big).
\end{align*}
\end{proof}

%\subsubsection{Application of Proposition \ref{prop: Ultimately uniqueness of Stokes data} to Stokes Data}
%\todo{I am slightly unsure where this section should be -- I expect that much of it should be in S4.  I also feel I am getting very unclear and I should write this out again}

\subsubsection{All roots in a plane}

%We first consider the case of two Stokes lines crossing labelled by roots $\alpha$ and $\beta$ crossing:

%\todo{say why nilpotent}

%Let $U_{\alpha, \beta}$ be the unipotent subgroup generated by $U_{\alpha}$ and $U_{\beta}$.  Then according to diagram [\todo{specify diagram}]

%we have that given initial Stokes data, $S_{\alpha}^{in}$ and $S_{\beta}^{in}$ applying the inverse of the map in proposition \ref{prop: Ultimately uniqueness of Stokes data} gives the Stokes factors on the outgoing lines.

%Furthermore the Stokes factors on the lines labelled by $\alpha$ and $\beta$ in the diagram remain unchanged because for the line labelled by $\alpha$ the map $U_{\alpha, \beta}$ .  The case of the line labelled by $\beta$ is completely analogous.

In Section \ref{sec: Cameral Networks}, we will introduce spectral networks. These consist of oriented curves on an algebraic curve, which switch order when they intersect. Moreover, in Section \ref{sec: flat Donagi Gaitsgory}, we associate unipotent automorphisms to each oriented curve segment. Here we are interested in how these unipotent automorphisms change when the curves switch order. 
Consider, then, an intersection of $k$ curves, labeled by a maximal planar, convex, set of roots.
The incoming curves are ordered according to the planar order (defined in \ref{def:convex_hulls}) of their labels. The outgoing curves have reversed order; see Figure \ref{fig:rays_reverse}.

\begin{figure}
    \centering
    \includegraphics[scale = 0.7]{images/rays_reverse.png}
    \caption{Intersection corresponding to maximal convex set of roots.}
    \label{fig:rays_reverse}
\end{figure}

Then we are interested in the specialization of the formulas in Lemma \ref{lem:sort_sigma} to the case $\sigma(i) = k-i$. For this choice of $\sigma$, the constants $c_{ij}$ in equations \ref{eq:sort_A2} - \ref{sort_G2} are all 1.

\begin{example}[Cecotti--Vafa Wall Crossing Formula]
Consider a Lie algebra $\fr g$ of ADE type. Then $k \leq 3$. In the case $k=3$, the specialization of \ref{eq:sort_A2} to $\sigma(i) = 3-i$ is:
\begin{equation}
\label{eq:CV_A2}
\exp(X_1) \exp(X_2) \exp(X_3) 
= 
\exp\big(X_3\big) 
\exp\big(X_2 + [X_1,X_3]\big) 
\exp\big(X_1\big).
\end{equation}
\end{example}

\begin{example}[B2 analogue of Cecotti--Vafa Wall Crossing Formula]
In the B2 case, the specialization of \ref{sort_B2} to $\sigma(i) = 4-i$ is:
\begin{align}
\begin{split}
\label{eq:CV_B2}
\exp&(X_1) \exp(X_2) \exp(X_3) \exp(X_4)
= 
\\
&=
\exp\big(X_4\big)
\exp\big(X_3 + [X_1, X_4]\big) 
\exp\left(X_2 + [X_1,X_3] + \frac{1}{2}[X_1,X_4]^{[2]}\right) 
\exp\big(X_1\big).
\end{split}
\end{align}

\end{example}

\begin{example}[G2 analogue of Cecotti--Vafa Wall Crossing Formula]
In the G2 case, the specialization of \ref{sort_G2} to $\sigma(i) = 6-i$ is:
\begin{align}
\begin{split}
\label{eq:CV_G2}
\exp&(X_1) \exp(X_2) \exp(X_3) \exp(X_4) \exp(X_5) \exp(X_6)
= 
\\
=&
\exp\big(X_6\big)
\exp\big(X_5 + [X_1,X_6]\big)
\\
&
\exp\left(
X_4 + [X_2,X_6] + [X_3,X_5] 
+ \frac{1}{2} \big[ [X_1,X_6]^{[2]},X_5 \big]
+ \frac{1}{6} \big[ [X_1,X_6],[X_1,X_6]^{[2]} \big]
\right)
\\
&
\exp\left(X_3 + [X_1, X_5]
+ \frac{1}{2} [X_1,X_6]^{[2]}\right) 
\exp\left(X_2 + [X_1,X_3] + \frac{1}{6}[X_1,X_6]^{[3]}\right) 
\exp\big(X_1\big).
\end{split}
\end{align}

\end{example}

%\subsubsection{All outgoing rays on single arc}

%It is clear that the above procedure can generalize to the following case 

%\todo{specify all Stokes rays need to be separated +++ }

%\todo{diagram illustrating the problem}

\subsubsection{Rays Not Separated, simply laced case}

\begin{lemma}[Faces and projection]
\label{lem:faces_projection}
Let $\Delta_{f}\subset \Delta$ be a face of the cone $\Delta$. The projection $p_f: \fu_{\Delta}\rightarrow \fu_{\Delta_{f}}$ with kernel $\oplus_{v\in \Phi\cap (\Delta\backslash \Delta_{f})}\fg_{v}$ is a morphism of Lie algebras.
\end{lemma}

\begin{proof}
We need to prove that $p_f\big([X_1,X_2]\big) = \big[p_f(X_1),p_f(X_2)\big]$, for all $X_1, X_2 \in \fr u_{\Delta}$. We analyze two cases.
\begin{itemize}
    \item If $X_1, X_2 \in \fu_{\Delta_f}$, then $[X_1, X_2] \in \fu_{\Delta_f}$, due to Lemma \ref{lem:roots_commutators_vanish}. So $p_f$ leaves each of $X_1, X_2, [X_1,X_2]$ unchanged.
    \item If at least one of $X_1, X_2$ is not in $\fu_{\Delta_f}$, then, using Lemma \ref{lem:roots_commutators_vanish} and the assumption that $\Delta_f$ is a face, either $[X_1, X_2] = 0$ or $[X_1, X_2] \not \in \fu_{\Delta_f}$. Thus, the equality $p_f\big([X_1,X_2]\big) = \big[p_f(X_1),p_f(X_2)\big]$ holds with both sides equal to 0.
\end{itemize}
\end{proof}

As a consequence:

\begin{lemma}
The map $U_{\Delta}\to U_{\Delta_{f}}$
which acts as the identity on $U_{\Delta_f}$ and sends every element not in $U_{\Delta_f}$ to $\id_{U_{\Delta_f}}$ is a Lie group homomorphism.
\end{lemma}

Let $\Delta$ be a cone.  Define $\fu_{\ker}$ as the kernel
\[
\fu_{\ker}\rightarrow \fu_{\Delta}\rightarrow \oplus_{\Delta_{i} face of \Delta}\fu_{\Delta_{i}}.\]
Note that this is Lie algebra by Lemma \ref{lem:faces_projection}.

\begin{conjecture}
If $\fg$ is simply laced then $dim(\fu_{Ker})\leq 1$.
\end{conjecture}

%\todo{Proof sketch -- FIX UP}Add the assumption that he number of one dimensional faces = the dimension of the cone.  Conjecture that it extends beyond this case.

%Assume the reverse, then there are two interior roots, by assumption these are $\sum_{i}a_{i}\alpha_{i}$ and $\sum_{i}b_{i}\alpha_{i}$, where $\alpha_{i}$ the roots on the one dimensional faces.  Interior means all $a_{i}, b_{i}\neq 0$.  Take $\gamma=\sum_{i}min(a_{i}, b_{i})\alpha_{i}$.  Take $\delta=\sum_{i}min(1, a_{i}-min(a_{i}, b_{i}))\alpha_{i}$, then $\delta, \gamma, \gamma+\delta, \gamma-\delta$ are four planar roots.  This means we have a two dimensional sub root system of type $B2$ or $G2$.  This contradicts simply laced assumption.

\begin{remark}
Note that the conjecture is clearly does not extend to the case where $\fg$ is not simply laced, as can be seen by considering the case where $\Delta$ is two dimensional.
\end{remark}

%\begin{proposition}[Stokes data where we do not necessarily have all outgoing rays on an arc]

%\end{proposition}

%\todo{Use T-equivariance to prove that we have the necessary maps in S5.3! (except the lines produced at ramification points)}





\subsubsection{Generalization to non-planar convex sets}

Any convex set of roots is contained in $\Phi_+$, for an appropriate choice of polarization $\Phi = \Phi_+ \coprod \Phi_-$. We prove the necessary results in the case that the convex set is $\Phi_+$ itself, and then show how this implies the results for any other convex set.

\begin{definition}
A \textbf{convex order} on $C \subset \Phi_+$ is a total order such that, if $\gamma = \alpha + \beta$ with $\alpha, \beta, \gamma \in C$, then either $\alpha < \gamma < \beta$, or $\alpha > \gamma > \beta$.
\end{definition}

\begin{lemma}[Lemma 2.1 in \cite{mcnamara2012}]
For any reductive $\fg$ and any polarization of $\Phi$, there exists a convex order on $\Phi_+$.
\end{lemma}

\begin{proof}
It suffices to give an argument for simple $\fg$, because roots from distinct simple summands don't interact.

A constructive proof for simple $\fg$ is given in Lemma 2.1 of \cite{mcnamara2012}; here we just sketch the construction of loc. cit. Let $\{\alpha_1, \dots, \alpha_d\}$ denote the simple roots for the chosen polarization, and $\{s_1, \dots, s_d\} \subset W$ the corresponding reflections. Let $w_0 \in W$ be the longest element for this polarization, and choose a decomposition:
\[
w_0 = s_{i_1} \dots s_{i_n}.
\]
Then define, for all $1 \leq j \leq n$:
\[
\gamma_j := s_{i_n} \dots s_{i_{j+1}} \alpha_{i_j}.
\]
Then $\{\gamma_1, \dots, \gamma_n\} = \Phi_+$, and the subscript provides a convex order. \todo{Details of Why?}
\end{proof}

This allows us to prove:

\begin{lemma}
\label{lem:convex_sort_sigma}
Let $\{\gamma_1, \dots, \gamma_n\}$ be a convex ordered enumeration of $\Phi_+$.
For every $\sigma \in S_n$, there is an isomorphism of schemes $\sort_\sigma$ which commutes with the multiplication maps:
\[
\begin{tikzcd}
U_{\gamma_{\sigma(1)}} \times \dots \times U_{\gamma_{\sigma(n)}}
\arrow{r}{m}
\arrow{d}{\sort_\sigma}
&
U_{\Phi_+}
\\
U_{\gamma_1} \times \dots \times U_{\gamma_n}
\arrow{ur}{m'}
&
\end{tikzcd}
\]
\end{lemma}

\begin{proof}
The construction of $\sort_\sigma$ is the same as in the planar case, but using a convex order rather than a planar order. This gives a map:
\[
\Big(
\exp \big( X_{\sigma(1)}\big),
\dots ,
\exp \big( X_{\sigma(n)}\big)
\Big)
\mapsto 
\Big(
\exp \big( X_1 + \text{junk}_1 \big),
\dots ,
\exp \big( X_n + \text{junk}_n \big)
\Big) .
\]
Here $\text{junk}_i$ is some linear combination of iterated Lie brackets of $X_1, \dots, X_n$.

It remains to show that $\sort_\sigma$ is invertible. The argument is by induction on the height of a positive root. If the expansion of $\gamma \in \Phi_+$ in the basis of simple roots is:
\[
\gamma = \sum_{i=1}^d a_i \alpha_i , \; a_i \in \N ,
\]
we define the height $h(\gamma) = \sum_{i=1}^d a_i$.

Note that $h(\gamma_1 + \gamma_2) = h(\gamma_1) + h(\gamma_2)$. Consequently, $\text{junk}_i$ only depends on those $X_j$ with $h(\gamma_j) < h(\gamma_i)$. From the output of $\sort_\sigma$, we can uniquely recover the inputs $X_1, \dots, X_n$ in increasing order of the height of the corresponding root.
\end{proof}

\begin{proposition}
\label{prop:convex_mult_iso}
Let $\{\gamma_1, \dots, \gamma_n\}$ be an enumeration of $\Phi_+$ in any order. Then the multiplication map is an isomorphism of schemes:
\[
\begin{tikzcd}
U_{1} \times \dots \times U_{n}
\arrow{r}{m}
&
U_{\Phi_+}
\end{tikzcd}
\]
\end{proposition}

\begin{proof}
It suffices to prove this if $\{\gamma_1, \dots, \gamma_n\}$ are in a convex order. Otherwise we compose with the isomorphism $\sort_\sigma$.

For the convex order, surjectivity follows by taking $u \in U_{\Phi_+}$, regarding it as a word in elements of $U_1, \dots, U_n$, and using twisted transpositions and contractions to rewrite the word as a tuple $(u_1, \dots, u_n) \in U_1 \times \dots \times U_n$. This is the same as the construction of $\sort_\sigma$.\todo{Be clearer about why the convex order means that this is a finite process!}

Injectivity is proved by starting with two tuples such that:
\[
m(u_1, \dots, u_n) = m(u_1', \dots, u_n') .
\]
Then:\todo{In the above we have defined $m$ as a function taking in $n$ inputs -- below you put in two inputs -- you should presumably just be taking the normal multiplication in the group!}
\[
m({u_1'}^{-1},u_1) = m(u_2', \dots, u_n') \big(m(u_2, \dots, u_n)\big)^{-1}.
\]
The LHS is an element of $U_1$. Since we assumed that $\{\gamma_1, \dots, \gamma_n\}$ are in convex order, $\fu_{\gamma_2, \dots, \gamma_n}$ is closed under the Lie bracket\todo{and hence we get a subgroup $U_{\gamma_{1}...\gamma_{n}}$ -- explain what this is!}. Then the RHS is an element of $U_{\gamma_2, \dots, \gamma_n}$. But $U_1 \cap U_{\gamma_2, \dots, \gamma_n} = \{\id\}$, which shows that $u_1 = u_1'$. Iterating on this procedure, we obtain that $(u_1, \dots, u_n) = (u_1', \dots, u_n')$. 
\end{proof}

Assume now that $C \subset \Phi_+$ is a subset such that $\Conv^\N_C = C$. (This is a necessary and sufficient condition for $\fu_C$ to be closed under the Lie bracket.\todo{clumsy wording}) Any convex order on $\Phi_+$ restricts to a convex order on $C$. Therefore the construction of $\sort_\sigma$ can proceed just as in the case of $\Phi_+$. Moreover, the same argument using induction on height proves that $\sort_\sigma$ is invertible. Therefore Lemma \ref{lem:convex_sort_sigma} and Proposition \ref{prop:convex_mult_iso} hold if we replace $\Phi_+$ with $C$.  \todo{Make this into a proposition}



\subsubsection{Take three}

\begin{proposition}
\label{prop:mult_iso}
Let $C \subset \Phi$ be a convex subset such that $C = \Conv_C^\N$. Then multiplication gives an isomorphism of schemes:
\[
\prod_{\gamma \in C} U_{\gamma}
\overset{M}{\longrightarrow}
U_C ,
\]
for any ordering of the product on the left hand side.
\end{proposition}

\begin{proof}
We use the Baker-Campbell-Hausdorff formula:
\[
\exp(X) \exp(Y) 
= 
\exp \left( X + Y + \frac{1}{2}[X,Y] + \dots \right) ,
\]
where the dots indicate higher order iterated Lie brackets of $X$ and $Y$. We only need this formula for the case when each of $X$, $Y$ spans a root space of $\fg$. Due to Lemma \ref{lem:roots_commutators_vanish} and the convexity assumption, there are only finitely many nonzero iterated Lie brackets in this case.

For all $\gamma \in C$, let $X_\gamma \in \fu_\gamma$. Applying the Baker-Campbell-Hausdorff formula iteratively, we obtain:
\[
\prod_{\gamma \in C} \exp(X_\gamma) 
= 
\exp \left( \sum_{\gamma \in C} (X_\gamma + \text{junk}_\gamma) \right) ,
\]
where $\text{junk}_\gamma$ is the sum of all iterated Lie brackets which belong to the root space $\fu_\gamma$.

It follows that we have a commutative diagram of schemes:
\[
\begin{tikzcd}
\prod_{\gamma \in C} U_{\gamma} 
\arrow{r}{M}
&
U_C
\\
\bigoplus_{\gamma \in C} \fu_\gamma
\arrow{u}{\prod_{\gamma \in C} \exp }
\arrow{r}{m}
&
\fu_C ,
\arrow[swap]{u}{\exp}
\end{tikzcd}
\]
where $m$ is the map:
\begin{equation}
\label{eq:mult_bijective}
(X_\gamma)_{\gamma \in C} 
\longmapsto
(X_\gamma + \text{junk}_\gamma)_{\gamma \in C} .
\end{equation}
Since the vertical arrows are isomorphisms of schemes, it suffices to prove that $m$ is invertible. We will argue by induction on the height of $\gamma \in C$, so let us recall the concept of height of a root. 

Since $C$ is convex, there exists a polarization $\Phi = \Phi_+ \coprod \Phi_-$ such that $C \subset \Phi_+$. Let $\{\alpha_1, \dots, \alpha_d\}$ denote the simple roots with respect to this polarization, and recall that the simple roots are a basis for the root system. Then all $\gamma \in C$ can be written uniquely as:
\[
\gamma = \sum_{i=1}^d n_i \alpha_i ,\; n_i \in \N .
\]
Then we define the height of $\gamma$ as $ht(\gamma) = \sum_{i=1}^d n_i$. In particular, $ht(\gamma_1) + ht(\gamma_2) = ht(\gamma_1 + \gamma_2)$. 

Using Lemma \ref{lem:roots_commutators_vanish}, we obtain that, if $[X_{\beta},X_{\delta}] \in \fu_{\gamma}$, then $ht(\beta), ht(\delta) < ht(\gamma)$. Generalizing, if an iterated Lie bracket involving $X_{\beta}$ belongs to $\fu_\gamma$, then $ht(\beta) < ht(\gamma)$. In other words, $\text{junk}_\gamma$ only depends on those $X_{\beta}$ with $ht(\beta) < ht(\gamma)$.

The inductive argument is as follows. Assume we know $X_\beta$ for all $\beta \in C$ such that $ht(\beta) < ht(\gamma)$. These determine $\text{junk}_\gamma$, so we can recover $X_\gamma$ uniquely from the output of \ref{eq:mult_bijective}.
\end{proof}

\begin{example}
For $\fg = \fr{sl}_3$, choose a polarization so that the positive root spaces correspond to upper-triangular matrices. We have the explicit formula:
\begin{align*}
\left( \begin{array}{ccc}
    1 & a & 0 \\
    0 & 1 & 0 \\
    0 & 0 & 1
\end{array}
\right)
\left( \begin{array}{ccc}
    1 & 0 & c \\
    0 & 1 & 0 \\
    0 & 0 & 1
\end{array}
\right)
\left( \begin{array}{ccc}
    1 & 0 & 0 \\
    0 & 1 & b \\
    0 & 0 & 1
\end{array}
\right)
&=
\left( \begin{array}{ccc}
    1 & a & c+ab \\
    0 & 1 & b \\
    0 & 0 & 1
\end{array}
\right)
\\
= \exp 
&
\left( \begin{array}{ccc}
    0 & a & c + ab/2 \\
    0 & 0 & b \\
    0 & 0 & 0
\end{array}
\right)
\end{align*}
The map $(a,b,c) \mapsto (a, b , c+ ab/2)$ is clearly invertible.
\end{example}

We remark that Proposition \ref{prop:mult_iso} is really a statement about root spaces. If we use a basis for $\fg$ that is not compatible with the root space decomposition, then the result need not be true.

\begin{example}
Let $\fg = \fr{sl}_3$, and choose the following basis for the Lie subalgebra of strictly upper triangular matrices:
\[
\left( \begin{array}{ccc}
    0 & 1 & 1 \\
    0 & 0 & 0 \\
    0 & 0 & 0
\end{array}
\right),
\hspace{1cm}
\left( \begin{array}{ccc}
    0 & 0 & 0 \\
    0 & 0 & 1 \\
    0 & 0 & 0
\end{array}
\right),
\hspace{1cm}
\left( \begin{array}{ccc}
    0 & 1 & -1 \\
    0 & 0 & 0 \\
    0 & 0 & 0
\end{array}
\right).
\]
Then:
\begin{align*}
\left( \begin{array}{ccc}
    1 & a & a \\
    0 & 1 & 0 \\
    0 & 0 & 1
\end{array}
\right)
\left( \begin{array}{ccc}
    1 & 0 & 0 \\
    0 & 1 & b \\
    0 & 0 & 1
\end{array}
\right)
\left( \begin{array}{ccc}
    1 & c & -c \\
    0 & 1 & 0 \\
    0 & 0 & 1
\end{array}
\right)
=&
\left( \begin{array}{ccc}
    1 & a+c & a-c + ab \\
    0 & 1 & b \\
    0 & 0 & 1
\end{array}
\right).
\end{align*}
Elements of the form:
\[
\left( \begin{array}{ccc}
    1 & x & z \\
    0 & 1 & y \\
    0 & 0 & 1
\end{array}
\right)
\]
with $y = -2$ and $x \neq -z$ form a codimension 1 locus not in the image of the multiplication map.
\end{example}



\subsubsection{A smorgasbord of Stokes factors}

In this part of the section, we obtain some corollaries of Proposition \ref{prop:mult_iso}, in the setting of Stokes factors associated to Stokes curves. We fix a convex set of roots $C$ such that $C = \Conv_C^{\N}$. We consider an intersection of Stokes curves, where there's one outgoing curve for every $\gamma \in C$; the incoming curves are a subset of the outgoing ones, and we let $C_{in} \subset C$ denote the corresponding set of roots.
The following is the simplest scenario.

\begin{corollary}
\label{cor:stokes_sector}
Assume that the outgoing curves are constrained to a sector of the plane with central angle $< \pi$; the situation is depicted in Figure \ref{fig:outgoing_sector}.

\begin{figure}
    \centering
    \includegraphics{stokes_around_joint.png}
    \caption{Outgoing curves in a sector with central angle $<\pi$.}
    \label{fig:outgoing_sector}
\end{figure}

Then there is a morphism of schemes:
\begin{align*}
\label{eq:stokes_in_to_out}
\prod_{\gamma \in C_{in}} U_\gamma 
&\to 
\prod_{\gamma \in C} U_\gamma  ,
\\
(u_\gamma)_{\gamma \in C_{in}}
&\mapsto 
(u'_\gamma)_{\gamma in C} ,
\end{align*}
where the products are taken in the order in which curves lie in the plane, such that:
\[
\prod_{\gamma \in C_{in}} u_\gamma 
=
\prod_{\gamma \in C} {u_{\gamma}'}.
\]
\end{corollary}

\begin{proof}
Let $m_{in} : \prod_{\gamma \in C_{in}} U_\gamma \to U_{C}$ be the multiplication map. Then the desired morphism is the composition:
\[
\begin{tikzcd}
\prod_{\gamma \in C_{in}} U_\gamma
\arrow{r}{m_{in}}
&
U_{C}
\arrow{r}{m^{-1}}
& 
\prod_{\gamma \in C} U_\gamma .
\end{tikzcd}
\]
The map $m^{-1}$ exists because of Proposition \ref{prop:mult_iso}.
\end{proof}

In the remainder of the section, we show that we can remove the assumption that the outgoing curves lie in a sector of central angle $< \pi$.

\begin{corollary}
\label{cor:stokes_in_to_out_mixed}
\end{corollary}



\begin{example}
\label{eg:A3_joint}
\todo{Write the example of the A3 joint.}
\end{example}
